JDEC: JPEG Decoding via Enhanced Continuous Cosine Coefficients

We propose a practical approach to JPEG image decoding, utilizing a local implicit neural representation with continuous cosine formulation. The JPEG algorithm significantly quantizes discrete cosine transform (DCT) spectra to achieve a high compression rate, inevitably resulting in quality degradation while encoding an image. We have designed a continuous cosine spectrum estimator to address the quality degradation issue that restores the distorted spectrum. By leveraging local DCT formulations, our network has the privilege to exploit dequantization and upsampling simultaneously. Our proposed model enables decoding compressed images directly across different quality factors using a single pre-trained model without relying on a conventional JPEG decoder. As a result, our proposed network achieves state-of-the-art performance in flexible color image JPEG artifact removal tasks. Our source code is available at https://github.com/WooKyoungHan/JDEC.

==> sec/0_abstract.tex <==
\begin{abstract}
% The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
% Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
% The abstract is to be in 10-point, single-spaced type.
% Leave two blank lines after the Abstract, then begin the main text.
% Look at previous \confName abstracts to get a feel for style and length. direct decoding 

% We propose an implicit neural representation that restores JPEG images by estimating discrete cosine transform (DCT) spectra. The JPEG, the most commonly used lossy compression algorithm, is designed based on the insight that the human visual system has a limited ability to distinguish high-frequency components. In order to achieve a high compression rate, the JPEG algorithm should significantly quantize DCT spectra. Therefore, recovering high-quality images is identical to the dequantization of spectra. Not only do we employ the recent novel de-quantization neural representation to DCT spectra, but we apply the upsampling mechanism for the color contrast, as well. As a result, our proposed network achieves state-of-the-art performance in color image JPEG artifact removal tasks.
% We propose a local implicit neural representation that restores JPEG images by formulating discrete cosine transform (DCT) spectra. The JPEG, the most commonly used lossy compression algorithm, is designed based on the insight that the human visual system has a limited ability to distinguish high-frequency components. The JPEG algorithm should significantly quantize DCT spectra to achieve a high compression rate. Therefore, recovering high-quality images is identical to the dequantization of spectra. We jointly estimate de-quantized spectra and frequency with a deep block transform. Our method implies dequantization and upsampling mechanisms by formulating features to the local DCT function. As a result, our proposed network achieves state-of-the-art performance in flexible color image JPEG artifact removal tasks.

% We propose a local implicit neural representation that restores JPEG images by formulating discrete cosine transform (DCT) spectra. We jointly estimate de-quantized spectra and frequency with a deep block transform.  
%The JPEG is designed with the understanding that the human visual system has a limitation in distinguishing high-frequency components. 
% We propose an innovative approach to JPEG image decoding utilizing a local implicit neural representation to reconstruct high-quality spectral information. The JPEG algorithm significantly quantizes discrete cosine transform (DCT) spectra to achieve a high compression rate. To improve the quality of JPEG images, we take advantage of a transformer architecture with high-frequency component estimation. The suggested architecture allows us to work with the distorted spectral data as input and decode the compressed images without degradation. Our approach involves dequantization and upsampling features by leveraging local DCT formulations. As a result, our proposed network achieves the state-of-the-art performance in flexible color image JPEG artifact removal tasks.
% Therefore, decoding high-quality images involves recovering spectra. We utilize a transformer architecture to enhance JPEG images by taking distorted spectral data as input. The JPEG algorithm significantly quantizes DCT spectra to achieve a high compression rate.  to reconstruct high-quality images.

We propose a practical approach to JPEG image decoding, utilizing a local implicit neural representation with continuous cosine formulation. The JPEG algorithm significantly quantizes discrete cosine transform (DCT) spectra to achieve a high compression rate, inevitably resulting in quality degradation while decoding a JPEG image.  We have designed a continuous cosine spectrum estimator to address the quality degradation issue that restores the distorted spectrum. By leveraging local DCT formulations, our network has the privilege to exploit dequantization and upsampling simultaneously. Our proposed model enables decoding compressed images directly across different quality factors using a single pre-trained model without relying on a conventional JPEG decoder. As a result, our proposed network achieves state-of-the-art performance in flexible color image JPEG artifact removal tasks. 
% It is inevitable to encounter quality degradation during the decoding of a JPEG image.
% To improve the quality of JPEG images, 
% By learning a function of block coordinates, our proposed model is able to decode JPEG images across various quality factors using a single pretrained model. 
%while considering the overall quality factor. 
 % The proposed architecture lets us accept distorted spectral data as input and decode compressed images while mitigating quality degradation.
 % The proposed architecture enables us to decode compressed images while minimizing quality degradation, even when distorted spectral data is given as input.
% Our approach realizes dequantization and upsampling by leveraging local DCT formulations.

%Source codes are included in the supplementary material.
%%%%%%%%%DR Jaedeock comments

%We propose an innovative method for JPEG decoding, employing a local implic`it neural representation to effectively reconstruct high-quality (?) spectral information. 
% The JPEG encoder involves quantizing the discrete cosine transform (DCT) spectra to achieve high compression rates, yet significantly distorting the spectra of the resulting image.
% Thus, it is inevitable to encounter a degradation in quality when decoding the JPEG image.
% To alleviate the quality degradation in decoding, we .... 
% (2~3 sentences to explain our work)
% As a result, our proposed network achieves the state-of-the-art performance in flexible color image JPEG artifact removal tasks (number?).
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}\label{sec:intro}



 

\ \ \ Within the dynamic evolution of high-efficiency image compression, it is notable that JPEG \cite{jpegstandard} maintains a pivotal position. JPEG, renowned for its compatibility and standardization, is the most famous image coder-decoder (CODEC) among conventional lossy compression methods. Therefore, a high-quality JPEG decoder applies to all existing compressed JPEG files. JPEG reduces file size through downsampling color components and quantizing the discrete cosine transform (DCT) spectra, which leads to a complicated loss of image information and distortion. Consequently, the design of a high-quality JPEG decoder presents a dual challenge: 1) the restoration of complex losses from the JPEG encoder and 2) the modeling of a network that employs a spectrum as an input and its image as an output.



%Consequently, solving an inverse problem stemming from JPEG compression presents a significant challenge, and the design of a high-quality decoder involves addressing this complex task.
 
% As the demand for high-efficiency image compression has grown, learning-based compression techniques have been actively researched. Despite this trend, JPEG remains the most widely used algorithm due to its cost-effectiveness and computational efficiency. JPEG is a prominent representative among traditional lossy compression techniques and distorts images based on the insight that the human eye is less sensitive to high-frequency components and less responsive to color variations. 
\begin{figure}[t]
\centering
\includegraphics[width = 3.2in]{Fig/1_Intro/Fig_1_ver_3_03.png}
\vspace{-8pt}
\caption{\textbf{Overall concept of proposed JPEG decoding} Instead of using a conventional JPEG decoder to refine the high-quality (HQ) image from the low-quality (LQ) image, our JDEC directly decodes the LQ spectrum by learning a continuous spectrum.}
\label{fig:concept}
\vspace{-15pt}
\end{figure}  

\begin{figure*}[t]
\footnotesize
\centering
% \includegraphics[height = 1.5in,width = 3.2in]{Fig/1_Intro/I_wish_Demo_Here.png}
\stackunder[2pt]{JPEG $(q=100)$}{\includegraphics[trim=0 170 330 50,clip,width = 2.03in]{Fig/Demo/jpeg_demo.png}}
\stackunder[2pt]{FBCNN \cite{fbcnn}}{\includegraphics[trim=0 170 330 50,clip,width = 2.03in]{Fig/Demo/fbcnn_demo.png}}
\stackunder[2pt]{\textbf{JDEC (\textit{ours})}}{\includegraphics[trim=0 170 330 50,clip,width = 2.03in]{Fig/Demo/ours_demo.png}} \\
\vspace{1mm}
{45.31 (dB) / 0.146 \qquad \qquad\qquad\qquad  \qquad \qquad 43.87 (dB) / 0.175 \qquad \qquad\qquad\qquad \qquad \qquad {\color{black}\textbf{46.80 (dB) / 0.139}}}
\vspace*{-7pt}
\caption{\textbf{Visual Demonstration at $q=100$} (PSNR (dB) $\uparrow$ / Bit-Error-Rate (BER) $\downarrow$) of decoding compressed image: JPEG (quality factor = 100), image enhancement approach \cite{fbcnn} predicted from JPEG image ($q=100$), and JDEC (\textit{ours}) predicted directly from a JPEG bit-stream. We highlight the occurrence of bit errors overlaid with green dots. }%Note that our network does not require the JPEG decoding process.
\vspace*{-12pt}
\label{fig:visual_demo}
\vspace{-4pt}
\end{figure*}



% Ehrlich \etal.'s approach \cite{qgac} utilizes a quantization matrix to flexibly retrieve all JPEG factors from given images, while Jiang \etal. \cite{fbcnn} extends a network with an additional classifier to predict quality factors and employs attention modules for image recovery.

Many deep neural networks (DNNs) have been proposed as promising solutions for the JPEG artifact removal \cite{arcnn,mwcnn,fbcnn,qgac,dncnn,idcn,dmcnn}. Most existing methods, such as \cite{arcnn,mwcnn}, are dedicated to specific quality factors, providing multiple models to cover JPEG compression. 
% Recently, \cite{qgac,fbcnn} proposed methods to solve the quality-dedicated problem by using quantization maps\cite{qgac} or estimating quality factor \cite{fbcnn}.  However, existing artifact removal networks typically receive the entire image as input despite most losses occurring in the spectrum, necessitating a JPEG decoder.
In recent studies \cite{qgac,fbcnn}, the quality-dedicated problem has been addressed through the utilization of quantization maps \cite{qgac} or the estimation of quality factors\cite{fbcnn}. 
The existing artifact removal networks commonly take the entire image as input, even though most losses occur in the spectrum. 
This limitation necessitates the use of a JPEG decoder.

 % Convolutional neural networks (CNNs) that take DCT spectra as an input have been discussed\cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning}.However, d

% Due to the characteristics of the JPEG algorithm, designing neural networks \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning} that take spectra as inputs is non-trivial. \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning} % An inverse discrete cosine transform (IDCT) is essential to convert frequency information into spatial information. IDCT is effectively achieved by formulating features using coordinate-based models, a.k.a. the implicit neural representation (INR) method.
Due to the characteristics of the JPEG algorithm, it is non-trivial to design a neural network that takes spectra as inputs \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning}. Park \etal \cite{rgbnomore} proposed a method of processing spectra to transformers.
%%%%%%
In the context of spectral processing, our approach extends beyond proposed classification networks \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning,rgbnomore} by leveraging the capabilities of the embedding strategy, paving the way for more effective decoding. The spectrum conversion aligns with recent advancements in implicit neural representation (INR), where methods adopting sinusoidal functions  \cite{Benbarka_2022_WACV,mildenhall2020nerf,sitzmann2019siren,lee2021local,lee2022learning,abcd} have demonstrated significant advancement across various tasks. 

%Not only does the sinusoidal representation enhance the network's performance \cite{Benbarka_2022_WACV,mildenhall2020nerf,sitzmann2019siren}, but it also proposes a way to learn sinusoidal components \cite{lee2021local,lee2022learning,abcd}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% While existing spectrum embedding methods \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning,rgbnomore} that primarily focus on classification, 
% we adopt the embedding idea to apply a transformer as the backbone of our network for decoding. 
% Recently, implicit neural representation (INR) methods adopting sinusoidal functions \cite{Benbarka_2022_WACV,mildenhall2020nerf,sitzmann2019siren,lee2021local,lee2022learning,abcd} have been proposed for various tasks. Not only does the sinusoidal representation enhance the network's performance \cite{Benbarka_2022_WACV,mildenhall2020nerf,sitzmann2019siren}, but it also proposes a way to learn sinusoidal components \cite{lee2021local,lee2022learning,abcd}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In the context of spectral processing, our approach extends beyond proposed classification networks \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning,rgbnomore} by leveraging the capabilities of the embedding strategy, paving the way for more effective decoding. The spectrum conversion aligns with recent advancements in implicit neural representation (INR), where methods adopting sinusoidal functions have demonstrated significant potential across various tasks.

% An inverse discrete cosine transform (IDCT) is essential to convert frequency information into spatial information. IDCT is effectively achieved by formulating features using coordinate-based models

%Using coordinate-based models, the  (INR) effectively decodes compressed JPEG code.

% To formulate a DCT transform with features, an implicit neural representation (INR) method is a reasonable approach. The work of Lee \etal \cite{lee2021local} formulates Fourier's transform with features and local coordinates of an image super-resolution INR. Not only does the Fourier representation enhance the network's performance, but it also suggests a way to learn dominant frequencies and amplitudes jointly.  To convert frequency information to spatial information, an inverse discrete cosine transform (IDCT) is necessary. To formulate a IDCT transform with features, coordinate-based models, a.k.a. an implicit neural representation (INR) method is a reasonable approach. 

% To formulate a DCT transform with features, an implicit neural representation (INR) method is a reasonable approach. The work of Lee \etal \cite{lee2021local} formulates Fourier's transform with features and local coordinates of an image super-resolution INR. Not only does the Fourier representation enhance the network's performance, but it also suggests a way to learn dominant frequencies and amplitudes jointly.

% In this paper, we design local INR, the Integrated Predictor of Enhanced Cosine coefficient (IPEC), to represent each 8$\times$8 patch, embedding each local coordinate with DCT formulation. IPEC utilizes local INR to solve complicated losses, quantization, and chroma-subsampling.

% **

% Recently, implicit neural representation (INR) methods have been spotlighted in various fields, such as image restoration. INR is a function that maps coordinates to specific signals with overfitting (e.g., view synthesis, images..). Learning local functions with encoded features makes INR take multiple images in image restoration tasks, such as single-image super-resolution. 

% \begin{figure}[t]
% \footnotesize
% \centering
% % \includegraphics[height = 1.5in,width = 3.2in]{Fig/1_Intro/I_wish_Demo_Here.png}
% \stackunder[2pt]{JPEG $(q=100)$}{\includegraphics[trim=0 170 330 50,clip,width = 1.05in]{Fig/Demo/jpeg_demo.png}}
% \hspace{-1mm}
% \stackunder[2pt]{FBCNN \cite{fbcnn}}{\includegraphics[trim=0 170 330 50,clip,width = 1.05in]{Fig/Demo/fbcnn_demo.png}}
% \hspace{-1mm}
% \stackunder[2pt]{\textbf{JDEC (\textit{ours})}}{\includegraphics[trim=0 170 330 50,clip,width = 1.05in]{Fig/Demo/ours_demo.png}} \\
% \hspace{-1mm}
% {45.31 (dB) / 0.146 \qquad  43.87 (dB) / 0.175 \qquad  {\color{black}\textbf{46.80 (dB) / 0.139}}}
% \vspace*{-7pt}
% \caption{\textbf{Visual Demonstration at $q=100$} (PSNR (dB) $\uparrow$ / Bit-Error-Rate (BER) $\downarrow$) of decoding compressed image: JPEG (quality factor = 100), image enhancement approach \cite{fbcnn} predicted from JPEG image ($q=100$), and JDEC (\textit{ours}) predicted directly from a JPEG bit-stream. We highlight the occurrence of bit errors overlaid with green dots. }%Note that our network does not require the JPEG decoding process.
% \vspace*{-12pt}
% \label{fig:visual_demo}
% \vspace{-4pt}
% \end{figure}



% Recently, an implicit neural representation (INR), which maps coordinates into signal values, shows promising performances in various tasks.
% The implicit neural networks have a spectral bias problem toward low frequencies, which makes INR hard to represent high-frequency components. Fortunately, several solutions are developed to relax the spectral bias. However, there is no INR approach for bit depth expansion problems.through the adaptive modeling of sinusoidal functions,
In this paper, we propose an advanced model, the JPEG Decoder with Enhanced Continuous cosine coefficients (JDEC), for retrieving high-quality images from compressed spectra. As an artifact removal network, our JDEC does not require a conventional JPEG decoder compared to existing methods shown in \cref{fig:concept}. JDEC captures the dominant frequency and its amplitude, thereby representing the high-quality spectrum through continuous cosine formulation (CCF). The CCF module estimates a continuous form of a given discrete cosine spectrum. The proposed model represents a considerable improvement in decoding JPEG bitstream. As shown in \cref{fig:visual_demo}, our JDEC decodes high-quality images with fewer bit errors than the original JPEG decoder.

% In this paper, we propose an innovative model, the Deep JPEG Decoder (DJ-12), for retrieving a high-quality image from its spectrum that is compressed with an arbitrary quality factor. By using a novel embedding method \cite{rgbnomore}, we utilize a robust transformer Swinv2\cite{Liu_2022_CVPR_swin2} as an encoder of the JDEC to extract features effectively.

% In this paper, we propose a novel model, the Arbitrary Bit-wise Coefficient model for De-quantization (ABCD), to recover missing bits from the randomly quantized LBD image to any HBD image. The proposed model addresses the spectral bias of INR and improves de-quantization quality through the use of an encoder to estimate the dominant phasors in the ground truth. As shown in \cref{fig:concept}, our encoder estimates the dominant phasors to mitigate the spectral bias of INR. Then, the model utilizes an INR to achieve arbitrary-bit reconstructions in the amplitude domain. Finally, a bit decoding step converts bit coefficients into HBD images by multiplying the bit-basis. The proposed model represents a significant advancement over previous de-quantization techniques with providing high flexibility and accuracy as it effectively recovers missing bits from randomly quantized inputs.

In summary, our main contributions are as follows:
\begin{itemize}
    \item We propose a local implicit neural representation that decodes JPEG files across various quality factors (QF) with continuous cosine spectra.
    
    \item We show that the suggested continuous cosine formulation module lets the network predict spectra highly correlated with the ground truth's spectrum.

    \item We demonstrate that our proposed method operates as a practical decoder, delivering superior image quality, including the generally used quality factor.
    %coordinate-based function, enabling upsampling. unlike other artifact removal methods 우리는 우리가 제안한 방법이 실용적인 디코더로 작동하며, 일반적으로 사용되는 품질 요소를 포함하여 JPEG의 최고 품질을 달성한다는 것을 시연합니다.
    % \item We propose an enhanced JPEG decoder that recovers images with arbitrary quality factors based on an implicit neural representation.
    % We demonstrate that our proposed method operates as a practical decoder, achieving the best quality of JPEG, including the generally used quality factor.

    % We demonstrate that our proposed approach operates effectively as a practical decoder, delivering superior image quality, including the commonly used quality factor.
    
    % \item We utilize the transformer as a backbone of our network by embedding the distorted spectrum.
    

\end{itemize}



==> sec/1_intro_camready.tex <==
\section{Introduction}\label{sec:intro}



 

\ \ \ Within the dynamic evolution of high-efficiency image compression, it is notable that JPEG \cite{jpegstandard} maintains a pivotal position. JPEG, renowned for its compatibility and standardization, is the most famous image coder-decoder (CODEC) among conventional lossy compression methods. Therefore, a high-quality JPEG decoder applies to all existing compressed JPEG files. JPEG reduces file size through downsampling color components and quantizing the discrete cosine transform (DCT) spectra, which leads to a complicated loss of image information and distortion. Consequently, the design of a high-quality JPEG decoder presents a dual challenge: 1) the restoration of complex losses from the JPEG encoder and 2) the modeling of a network that employs a spectrum as an input and its image as an output.



%Consequently, solving an inverse problem stemming from JPEG compression presents a significant challenge, and the design of a high-quality decoder involves addressing this complex task.
 
% As the demand for high-efficiency image compression has grown, learning-based compression techniques have been actively researched. Despite this trend, JPEG remains the most widely used algorithm due to its cost-effectiveness and computational efficiency. JPEG is a prominent representative among traditional lossy compression techniques and distorts images based on the insight that the human eye is less sensitive to high-frequency components and less responsive to color variations. 
\begin{figure}[t]
\centering
% \includegraphics[trim = 340 130 270 172,clip, width = 3.2in]{camreadyfig/Fig_1_ver_final.png}
\includegraphics[trim = 340 130 270 172,clip, width = 3.2in]{x2/jpeg/Fig_1_ver_final.jpg}
% \includegraphics[trim = 170 65 135 86,clip, width = 3.2in]{x2/x2/Fig_1_ver_final.png}
\vspace{-8pt}
\caption{\textbf{Overall concept of proposed JPEG decoding} Instead of using a conventional JPEG decoder to refine the high-quality (HQ) image from the low-quality (LQ) image, our JDEC directly decodes the LQ spectrum by learning a continuous spectrum.}
\label{fig:concept}
\vspace{-15pt}
\end{figure}  

% \begin{figure*}[t]
% \footnotesize
% \centering
% % \includegraphics[height = 1.5in,width = 3.2in]{Fig/1_Intro/I_wish_Demo_Here.png}
% \stackunder[2pt]{JPEG $(q=100)$}{\includegraphics[trim=0 170 330 50,clip,width = 2.03in]{Fig/Demo/jpeg_demo.png}}
% \stackunder[2pt]{FBCNN \cite{fbcnn}}{\includegraphics[trim=0 170 330 50,clip,width = 2.03in]{Fig/Demo/fbcnn_demo.png}}
% \stackunder[2pt]{\textbf{JDEC (\textit{ours})}}{\includegraphics[trim=0 170 330 50,clip,width = 2.03in]{Fig/Demo/ours_demo.png}} \\
% \vspace{1mm}
% {45.31 (dB) / 0.146 \qquad \qquad\qquad\qquad  \qquad \qquad 43.87 (dB) / 0.175 \qquad \qquad\qquad\qquad \qquad \qquad {\color{black}\textbf{46.80 (dB) / 0.139}}}
% \vspace*{-7pt}
% \caption{\textbf{Visual Demonstration at $q=100$} (PSNR (dB) $\uparrow$ / Bit-Error-Rate (BER) $\downarrow$) of decoding compressed image: JPEG (quality factor = 100), image enhancement approach \cite{fbcnn} predicted from JPEG image ($q=100$), and JDEC (\textit{ours}) predicted directly from a JPEG bit-stream. We highlight the occurrence of bit errors overlaid with green dots. }%Note that our network does not require the JPEG decoding process.
% \vspace*{-12pt}
% \label{fig:visual_demo}
% \vspace{-4pt}
% \end{figure*}



% Ehrlich \etal.'s approach \cite{qgac} utilizes a quantization matrix to flexibly retrieve all JPEG factors from given images, while Jiang \etal. \cite{fbcnn} extends a network with an additional classifier to predict quality factors and employs attention modules for image recovery.

Many deep neural networks (DNNs) have been proposed as promising solutions for the JPEG artifact removal \cite{arcnn,mwcnn,fbcnn,qgac,dncnn,idcn,dmcnn}. Most existing methods, such as \cite{arcnn,mwcnn}, are dedicated to specific quality factors, providing multiple models to cover JPEG compression. 
% Recently, \cite{qgac,fbcnn} proposed methods to solve the quality-dedicated problem by using quantization maps\cite{qgac} or estimating quality factor \cite{fbcnn}.  However, existing artifact removal networks typically receive the entire image as input despite most losses occurring in the spectrum, necessitating a JPEG decoder.
In recent studies \cite{qgac,fbcnn}, the quality-dedicated problem has been addressed through the utilization of quantization maps \cite{qgac} or the estimation of quality factors \cite{fbcnn}. 
% The existing artifact removal networks commonly take the decoded image as input, even though the encoded spectrum contains more information than the decoded image, according to the data processing inequality \cite{informationtheorybook}. The property is explained in \cref{sec:supp_dpi}.% E.G Chroma converter/  DCT
The existing artifact removal networks commonly take the decoded image as input, even though the encoded spectrum contains more information than the decoded image, according to the data processing inequality \cite{informationtheorybook}. The property is explained in the supplement material.% E.G Chroma converter/  DCT
%The existing artifact removal networks commonly take the entire image as input, even though most losses occur in the spectrum. This limitation necessitates the use of a JPEG decoder. (수정전)


 % Convolutional neural networks (CNNs) that take DCT spectra as an input have been discussed\cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning}.However, d

% Due to the characteristics of the JPEG algorithm, designing neural networks \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning} that take spectra as inputs is non-trivial. \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning} % An inverse discrete cosine transform (IDCT) is essential to convert frequency information into spatial information. IDCT is effectively achieved by formulating features using coordinate-based models, a.k.a. the implicit neural representation (INR) method.
Due to the characteristics of the JPEG algorithm, it is non-trivial to design a neural network that takes spectra as inputs \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning}. Park \etal \cite{rgbnomore} proposed a method of processing spectra to transformers.
%%%%%%
In the context of spectral processing, our approach extends beyond proposed classification networks \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning,rgbnomore} by leveraging the capabilities of the embedding strategy, paving the way for more effective decoding. The spectrum conversion aligns with recent advancements in implicit neural representation (INR), where methods adopting sinusoidal functions  \cite{Benbarka_2022_WACV,mildenhall2020nerf,sitzmann2019siren,lee2021local,lee2022learning,abcd} have demonstrated significant advancement across various tasks. 

%Not only does the sinusoidal representation enhance the network's performance \cite{Benbarka_2022_WACV,mildenhall2020nerf,sitzmann2019siren}, but it also proposes a way to learn sinusoidal components \cite{lee2021local,lee2022learning,abcd}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% While existing spectrum embedding methods \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning,rgbnomore} that primarily focus on classification, 
% we adopt the embedding idea to apply a transformer as the backbone of our network for decoding. 
% Recently, implicit neural representation (INR) methods adopting sinusoidal functions \cite{Benbarka_2022_WACV,mildenhall2020nerf,sitzmann2019siren,lee2021local,lee2022learning,abcd} have been proposed for various tasks. Not only does the sinusoidal representation enhance the network's performance \cite{Benbarka_2022_WACV,mildenhall2020nerf,sitzmann2019siren}, but it also proposes a way to learn sinusoidal components \cite{lee2021local,lee2022learning,abcd}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In the context of spectral processing, our approach extends beyond proposed classification networks \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning,rgbnomore} by leveraging the capabilities of the embedding strategy, paving the way for more effective decoding. The spectrum conversion aligns with recent advancements in implicit neural representation (INR), where methods adopting sinusoidal functions have demonstrated significant potential across various tasks.

% An inverse discrete cosine transform (IDCT) is essential to convert frequency information into spatial information. IDCT is effectively achieved by formulating features using coordinate-based models

%Using coordinate-based models, the  (INR) effectively decodes compressed JPEG code.

% To formulate a DCT transform with features, an implicit neural representation (INR) method is a reasonable approach. The work of Lee \etal \cite{lee2021local} formulates Fourier's transform with features and local coordinates of an image super-resolution INR. Not only does the Fourier representation enhance the network's performance, but it also suggests a way to learn dominant frequencies and amplitudes jointly.  To convert frequency information to spatial information, an inverse discrete cosine transform (IDCT) is necessary. To formulate a IDCT transform with features, coordinate-based models, a.k.a. an implicit neural representation (INR) method is a reasonable approach. 

% To formulate a DCT transform with features, an implicit neural representation (INR) method is a reasonable approach. The work of Lee \etal \cite{lee2021local} formulates Fourier's transform with features and local coordinates of an image super-resolution INR. Not only does the Fourier representation enhance the network's performance, but it also suggests a way to learn dominant frequencies and amplitudes jointly.

% In this paper, we design local INR, the Integrated Predictor of Enhanced Cosine coefficient (IPEC), to represent each 8$\times$8 patch, embedding each local coordinate with DCT formulation. IPEC utilizes local INR to solve complicated losses, quantization, and chroma-subsampling.

% **

% Recently, implicit neural representation (INR) methods have been spotlighted in various fields, such as image restoration. INR is a function that maps coordinates to specific signals with overfitting (e.g., view synthesis, images..). Learning local functions with encoded features makes INR take multiple images in image restoration tasks, such as single-image super-resolution. 

\begin{figure}[t]
\footnotesize
\centering
% \includegraphics[height = 1.5in,width = 3.2in]{Fig/1_Intro/I_wish_Demo_Here.png}
\stackunder[2pt]{JPEG $(q=100)$}{\includegraphics[trim=0 85 165 25,clip,width = 1.05in]{x2/x2/jpeg_demo.png}}
\hspace{-1mm}
\stackunder[2pt]{FBCNN \cite{fbcnn}}{\includegraphics[trim=0 85 165 25,clip,width = 1.05in]{x2/x2/fbcnn_demo.png}}
\hspace{-1mm}
\stackunder[2pt]{\textbf{JDEC (\textit{ours})}}{\includegraphics[trim=0 85 165 25,clip,width = 1.05in]{x2/x2/ours_demo.png}} \\
% {\includegraphics[trim=0 170 330 50,clip,width = 1.05in]{Fig/Demo/ours_demo.png}} \\
\hspace{-1mm}
{45.31 (dB) / 0.146 \qquad  43.87 (dB) / 0.175 \qquad  {\color{black}\textbf{46.80 (dB) / 0.139}}}
\vspace*{-7pt}
\caption{\textbf{Visual Demonstration at $q=100$} (PSNR (dB) $\uparrow$ / Bit-Error-Rate (BER) $\downarrow$) of decoding compressed image: JPEG (quality factor = 100), image enhancement approach \cite{fbcnn} predicted from JPEG image ($q=100$), and JDEC (\textit{ours}) predicted directly from a JPEG bit-stream. We highlight the occurrence of bit errors overlaid with green dots. }%Note that our network does not require the JPEG decoding process.
\vspace*{-15pt}
\label{fig:visual_demo}
\vspace{-4pt}
\end{figure}



% Recently, an implicit neural representation (INR), which maps coordinates into signal values, shows promising performances in various tasks.
% The implicit neural networks have a spectral bias problem toward low frequencies, which makes INR hard to represent high-frequency components. Fortunately, several solutions are developed to relax the spectral bias. However, there is no INR approach for bit depth expansion problems.through the adaptive modeling of sinusoidal functions,
In this paper, we propose an advanced model, the JPEG Decoder with Enhanced Continuous cosine coefficients (JDEC), for retrieving high-quality images from compressed spectra. As an artifact removal network, our JDEC does not require a conventional JPEG decoder compared to existing methods shown in \cref{fig:concept}. JDEC captures the dominant frequency and its amplitude, thereby representing the high-quality spectrum through continuous cosine formulation (CCF). The CCF module estimates a continuous form of a given discrete cosine spectrum. The proposed model represents a considerable improvement in decoding JPEG bitstream. As shown in \cref{fig:visual_demo}, our JDEC decodes high-quality images with fewer bit errors than the original JPEG decoder.

% In this paper, we propose an innovative model, the Deep JPEG Decoder (DJ-12), for retrieving a high-quality image from its spectrum that is compressed with an arbitrary quality factor. By using a novel embedding method \cite{rgbnomore}, we utilize a robust transformer Swinv2\cite{Liu_2022_CVPR_swin2} as an encoder of the JDEC to extract features effectively.

% In this paper, we propose a novel model, the Arbitrary Bit-wise Coefficient model for De-quantization (ABCD), to recover missing bits from the randomly quantized LBD image to any HBD image. The proposed model addresses the spectral bias of INR and improves de-quantization quality through the use of an encoder to estimate the dominant phasors in the ground truth. As shown in \cref{fig:concept}, our encoder estimates the dominant phasors to mitigate the spectral bias of INR. Then, the model utilizes an INR to achieve arbitrary-bit reconstructions in the amplitude domain. Finally, a bit decoding step converts bit coefficients into HBD images by multiplying the bit-basis. The proposed model represents a significant advancement over previous de-quantization techniques with providing high flexibility and accuracy as it effectively recovers missing bits from randomly quantized inputs.

In summary, our main contributions are as follows:
\begin{itemize}
    \item We propose a local implicit neural representation that decodes JPEG files across various quality factors (QF) with continuous cosine spectra.
    
    \item We show that the suggested continuous cosine formulation module lets the network predict spectra highly correlated with the ground truth's spectrum.

    \item We demonstrate that our proposed method operates as a practical decoder, delivering superior image quality, including the generally used quality factor.
    %coordinate-based function, enabling upsampling. unlike other artifact removal methods 우리는 우리가 제안한 방법이 실용적인 디코더로 작동하며, 일반적으로 사용되는 품질 요소를 포함하여 JPEG의 최고 품질을 달성한다는 것을 시연합니다.
    % \item We propose an enhanced JPEG decoder that recovers images with arbitrary quality factors based on an implicit neural representation.
    % We demonstrate that our proposed method operates as a practical decoder, achieving the best quality of JPEG, including the generally used quality factor.

    % We demonstrate that our proposed approach operates effectively as a practical decoder, delivering superior image quality, including the commonly used quality factor.
    
    % \item We utilize the transformer as a backbone of our network by embedding the distorted spectrum.
    

\end{itemize}



==> sec/2_related_work.tex <==
\section{Related Work}\label{sec:related}

% \begin{figure*}[t]
% \footnotesize
% \centering
% % \includegraphics[height = 1.5in,width = 3.2in]{Fig/1_Intro/I_wish_Demo_Here.png}
% \stackunder[2pt]{\includegraphics[trim=0 220 330 0,clip,width = 2.03in]{Fig/Demo/jpeg_demo.png}}{JPEG $(q=100)$}
% \stackunder[2pt]{\includegraphics[trim=0 220 330 0,clip,width = 2.03in]{Fig/Demo/fbcnn_demo.png}}{FBCNN\cite{fbcnn}}
% \stackunder[2pt]{\includegraphics[trim=0 220 330 0,clip,width = 2.03in]{Fig/Demo/ours_demo.png}}{\textbf{JDEC(Ours)}}
% \caption{\textbf{Visual Demonstration} of decoding compressed image: JPEG (quality factor = 0), image enhancement approach\cite{fbcnn}, and ours. Note that our network does not require the JPEG decoding process.}
% \vspace*{-15pt}
% \label{fig:rdcurve}
% \vspace{-4pt}
% \end{figure*}


 % with a 4:2:0 ratio \cite{jpegstandard}, equivalent to the 
\textbf{JPEG Background} According to Shannon's source coding theorem \cite{shannoncapacity}, a loss of image information is unavoidable to achieve high-efficiency compression.
The JPEG initiates the encoding process by decomposing an input RGB image to luminance and chroma components \cite{jpegstandard}. 
The chroma components are downsampled using the nearest neighbor method by a factor of $\times 2$. 
The JPEG subtracts the midpoint of the pixel value (=128) to images and divides it into $8\times8$ crops. Then, each crop is transformed into 2D-DCT \cite{ahmed1974discrete} spectra.
Following this, the encoder quantizes the spectrum of each block using a predefined quantization matrix depending on a quality factor $q$, and then the quantized spectrum is coded using Huffman coding. 
We illustrate the process of the JPEG encoder in \cref{fig:jpeg_process}.

Due to the nature of DCT, the energy of spectra is concentrated in low-frequency components. 
% All losses occur in the orange area of \cref{fig:jpeg_process}. 
% Most of losses occur in high-frequency components because the quantization matrix is a modified low-pass filter, and the chroma downsampling is equivalent to low-pass filtering. 
% The conventional decoder of the JPEG multiplies the quantization matrix to quantized spectra and transforms them into images. Therefore, all incurred losses, especially high-frequency components, are directly conveyed to the image. 
% Most distortion occurs in high-frequency components because the quantization matrix acts as a modified low-pass filter.
Since the quantization matrix treats high-frequency components more severely than low-frequency components, most distortions occur in the high-frequency components.
In the JPEG decoder, the quantization matrix is directly applied to the quantized spectra, transforming them into images. 
Consequently, all incurred losses, especially those in high-frequency components, are directly conveyed to the resulting image.

 % Zhang \etal \cite{dncnn} uses a residual approach to accelerate the training time and enhance the proposed network's performance.
\begin{figure}[t]
\footnotesize
\centering
\includegraphics[width = 3.4in]{Fig/3_Problemformulation/Fig_3_ver_2_02.png}
\caption{\textbf{Overall process of the JPEG encoder.} Luminance and chroma components are separated from an RGB image. Both components are converted to DCT spectra and quantized with a pre-defined quantization matrix (Q-map). All losses occur in the orange area.}%Chroma components are downsampled.
\vspace*{-15pt}
\label{fig:jpeg_process}
\vspace{-4pt}
\end{figure}
% Recovering highly compressed JPEG images is related to our work in the aspect of the high-quality decoder. 
\noindent{\bf JPEG Artifact Removal} 
To address the aforementioned problem, learning-based methods have enhanced the quality of a decoded image. 
Dong \etal \cite{arcnn} introduced a neural network that utilizes a super-resolution network \cite{srcnn} for JPEG artifact removal. 
Most of the proposed neural networks are dedicated to a specific quality factor \cite{cas-cnn,jpegrelateddedicated,arcnn,jpegrelatedwaveletcnn}. 
% <difficulties in generalize to jpeg decoder>
% methods that conduct multi-level JPEG artifact removal network have been proposed. 
To tackle the quality-dedicated issue, Jiang \etal \cite{fbcnn} proposed a method to estimate a quality factor, solving flexible JPEG artifact removal and handling a double JPEG artifact. 
However, the existing artifact removal methods take images as input, incorporating the conventional JPEG decoder before using their network. 
Recently, Bahat \etal \cite{bahat2021whatsin} proposed a novel method for JPEG decoding, which takes spectra as input. However, the proposed method does not consider color components with trainable decoding and does not recover high-quality factors.
% While the proposed method employs an image restoration approach and simplified chroma component recovery, asserting its status as a high-quality end-to-end decoder in restoring images for all quality factors is challenging.
% However, it is difficult to claim that the proposed method is a high-quality end-to-end decoder due to its image restoration approach: using inverse DCT, the inability to restore images for all quality factors, and the simplistic recovery of chroma components through spectral zero-padding.


% To operate a DNN as a decoder of the JPEG, algorithms should cover all of the quality factors as shown in \cref{fig:rdcurve}.
% \textbf{Background} According to Shannon's source coding theorem\cite{shannoncapacity}, a loss is inevitable to achieve high-efficiency compression. In this section, we briefly discuss the JPEG\cite{jpegstandard} encoding algorithm and summarize the essential role of the JPEG decoder. Let $\mathbf{I_{HQ}} \in \mathbb{R}^{H\times W \times 3}$ be a high-quality image. The JPEG encoder separates luminance components ($:=\mathbf{I_{Y}}\in \mathbb{R}^{H\times W \times 1}$) and chroma components ($:=\mathbf{I_{C}}\in \mathbb{R}^{H\times W \times 2}$) from RGB images. JPEG subsamples chroma components with a 4:2:0 ratio, equivalent to the {$\times 2$ nearest downsampling} ($\downarrow$ part in \cref{fig:jpeg_process}). Then, each component is divided into $8\times8$ crops ($\mathbf{I}=[I_{h,w}], (h,w\in \{0,1,\dots,7\}$) and transformed into 2D-DCT spectra $\mathbf{X} = [x_{u,v}]$ s.t.
% \begin{align}\label{eq:dct}
% \vspace*{-10pt}
%     \tiny
%     {x}_{u,v}:= \alpha_{u,v}\sum_{h,w}{I}_{h,w}\cos\left[ \frac{(2h+1)\pi u}{16} \right]\cos\left[ \frac{(2w+1)\pi v}{16} \right],
% \end{align}
% where $\alpha_{u,v}$ indicates weights for the orthonormality of the transform. Spectra divided with the pre-defined quantization map depending on the quality factor ($\mathbf{Q}:=[q_{u,v}]\in {\mathbb{N}^{8\times8}}$) and rounded s.t. 
% \begin{align}\label{eq:quantize_spectra}
% \vspace*{-15pt}
%     \Tilde{x}_{u,v} = \lfloor \frac{x_{u,v}}{q_{u,v}} \rceil q_{u,v}
% \vspace*{-15pt}
% \end{align}
% where $\lfloor \cdot \rceil$ is a round operation that maps to the nearest integer. The JPEG compresses $\mathbf{Q}$ and $\lfloor \cdot \rceil$ parts separately in the encoder part and calculates \cref{eq:quantize_spectra} in the conventional decoder part.
% To summarize this, the corrupted JPEG image $\tilde{\mathbf{I}}$ is 
% \begin{align}\label{eq:overall}
% \mathbf{\tilde{I}}
% \overset{\text{\cref{eq:dct}}}{\longleftrightarrow}& \left[ Q\mathbf{({X}_{Y})};Q\mathbf{({X}^{\downarrow}_{C})^{\uparrow}} \right] %Q\mathbf{({X}^{\downarrow}_{Cr}})^{\uparrow}
% \end{align}
% % \begin{align}
% % \mathbf{\tilde{I}} \sim& \left[\mathbf{\tilde{I}_Y}; \mathbf{\tilde{I}^{\uparrow}_{Cb}}; \mathbf{\tilde{I}^{\uparrow}_{Cr}}\right] \\
% % \overset{\text{\cref{eq:dct}}}{\longleftrightarrow}& \left[ Q\mathbf{({X}_{Y})};Q\mathbf{({X}^{\downarrow}_{Cb})};Q\mathbf{({X}^{\downarrow}_{Cr}}) \right] 
% % \end{align}
% where $Q(\cdot )$ is {\cref{eq:quantize_spectra}}, and $(\cdot)^{\uparrow}, (\cdot)^{\downarrow}$ indicates $\times2$ upsampling and downsampling in the spatial domain, respectively. Note that $\mathbf{\tilde{{X}}_{C}}\in \mathbb{R}^{\frac{H}{2}\times\frac{W}{2}\times2}$ while $\mathbf{\tilde{X}_Y} \in \mathbb{R}^{{H}\times{W}\times1}$. Therefore, designing the JPEG decoder should handle three issues: 1) covering all quality factors such as \cref{fig:rdcurve}, 2) retrieving losses driven from \cref{eq:overall}, 3) embedding $\mathbf{\tilde{X}_Y}, \mathbf{\tilde{{X}}_{C}}$ simultaneously where they have different size.

% % Thus, retrieving losses from JPEG compression is equal to reconstructing 1) quantization of spectra and 2) downsamples of chroma images.
\begin{figure*}[t]
\centering
% \includegraphics[trim=14 20 14 75,clip,width=7in]
\includegraphics[trim= 4 4 0 86,clip,width=7in]{Fig/3_Problemformulation/Fig_4_ver_3_main.png}
\caption{\textbf{Decoding a JPEG bitstream with the proposed JDEC.} JDEC consists of an encoder ($E_\varphi$) with group spectra embedding ($g_\phi$), a decoder ($f_\theta$), and continuous cosine formulation ($T_\psi$). Inputs of JDEC are as follows: compressed spectra ($\mathbf{\tilde{X}_Y},{\mathbf{\tilde{X}_C}}$), quantization map $\mathbf{Q}$. Note that our JDEC does not take ${\mathbf{\tilde{I}}}$ as an input. JDEC formulates latent features into a trainable continuous cosine coefficient as a function of block grid $\delta$ and forward to INR ($f_\theta$). Therefore, each $B\times B$ block shares the estimated continuous cosine spectrum. }
\label{Figmain}
\vspace{-12pt}
\end{figure*}

\noindent{\bf Learning in the Frequency domain} 
 In an image classification task, skipping a conventional JPEG decoding \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning} has been proposed, especially optimizing CNNs. Embedding techniques \cite{related_taking_freq_2018_fasterneural} tackle the size mismatch issue between luma and chroma components, such as upsampling chroma components before forwarding to a network and upsampling chroma features after forwarding to a shallow network. The proposed methods boost computation time without dropping the original performance. Recently, the approach adopting vision transformers \cite{vit2020ICLR} instead of CNNs has promising performance \cite{rgbnomore}. We adopt the proposed embedding method from \cite{rgbnomore} and modified \cite{Liu_2022_CVPR_swin2} SwinV2 transformer suitable for image decoding. 

 
 % Simply converting the input into a spectrum is insufficient for applying CNNs. There are two reasons for this; the first is that the color components are downsampled, and the second is due to the non-uniform energy density of the spectrum.


% The core component of the JPEG decoder is the Inverse DCT, which is a lossless linear function. From the perspective of a learning-based network, the decoder appears as if a single linear layer could replace them. However, several studies\cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning,decoderjpeglearningspectra} have demonstrated that this replacement is not easily attainable. Several approaches have been proposed to skip a conventional JPEG decoding in an image classification task \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning}, especially optimizing CNNs. Simply converting the input into a spectrum is insufficient for applying CNNs.
% There are two reasons for this; the first is that the color components are downsampled, and the second is due to the non-uniform energy density of the spectrum. Embedding techniques are suggested in \cite{related_taking_freq_2018_fasterneural}, such as upsampling chroma components before forwarding to a network and upsampling chroma features after forwarding to a shallow network. The suggested methods boost computation time without dropping the original performance.


% Since our work is the first in designing a learning-based JPEG decoder, 

% \noindent{\bf JPEG Artifact Removal} Recovering highly compressed JPEG images is related to our work in the aspect of the high-quality decoder. Recently, learning-based methods have enhanced the quality of a reconstructed image. Dong \etal \cite{arcnn} suggest the first neural network that utilizes a super-resolution network\cite{srcnn} for JPEG artifact removal. Zhang \etal \cite{dncnn} uses a residual approach to accelerate the training time and enhance the proposed network's performance. Since most of the proposed neural networks are dedicated to a specific quality factor \cite{cas-cnn,jpegrelateddedicated,arcnn,jpegrelatedwaveletcnn}, methods that conduct multi-level JPEG artifact removal network have been proposed. To tackle the aforementioned issue, Jiang \etal \cite{fbcnn} proposed a network with a quality factor estimator. The proposed method solves flexible JPEG artifact removal and handles a double JPEG artifact. To operate a DNN as a decoder of the JPEG, algorithms should cover all of the quality factors as shown in \cref{fig:rdcurve}.

% \noindent{\bf Implicit Neural Representation (INR)}  The coordinate-based multi-layer perceptrons(MLP) represent various continuous signals \cite{Occupancy_Networks,Local_Implicit_Grid_CVPR20,sitzmann2019siren,mildenhall2020nerf}. It has been proved that inserting sinusoidal functions into INR enhances the performance of network \cite{sitzmann2019siren,lee2021local,lee2022learning,abcd,mildenhall2020nerf,tancik2020fourfeat}. The recent image representing networks such as \cite{lee2021local,abcd} and \cite{sitzmann2019siren} were designed to tackle the spectral bias \cite{DBLP:conf/icml/RahamanBADLHBC19} which lead the network towards low-frequency components. Furthermore, the proposed methods demonstrated that frequencies\cite{lee2021local} and phasors\cite{abcd} are trainable components depending on images. The JPEG recovery is a complicated problem: quantization and upsampling (\cref{eq:overall}). In the aspect of signal processing, downsampling in the spatial domain is equivalent to low-pass filtering. Therefore, most high-frequency components vanish. We apply the estimation of the high-frequency components and reconstruct HQ images by adopting the \cref{eq:dct} as a local INR of images.


 % Recently, learning-based methods have enhanced the quality of a reconstructed image. Dong \etal \cite{arcnn} suggest the first neural network that utilizes a super-resolution network\cite{srcnn} for JPEG artifact removal. Zhang \etal \cite{dncnn} uses a residual approach to accelerate the training time and enhance the proposed network's performance. Since most of the proposed neural networks are dedicated to a specific quality factor \cite{cas-cnn,jpegrelateddedicated,arcnn,jpegrelatedwaveletcnn}, methods that conduct multi-level JPEG artifact removal network have been proposed. To tackle the aforementioned issue, Jiang \etal \cite{fbcnn} proposed a network with a quality factor estimator. The proposed method solves flexible JPEG artifact removal and handles a double JPEG artifact. To operate a DNN as a decoder of the JPEG, algorithms should cover all of the quality factors as shown in \cref{fig:rdcurve}.

% \begin{figure}[t]
% \centering
% \footnotesize
% \hspace{0.06mm}
% \stackunder[2pt]{\includegraphics[trim=0 0 0 0,clip,width=1.5in]{Fig/2_Relatedwork/Fig_3-1_ver_1_00.png}}{(a) Dynamic Range}
% \hspace{3mm}
% \stackunder[2pt]{\includegraphics[trim=0 0 0 0,clip,width=1.5in]{Fig/2_Relatedwork/Fig_3-2_ver_1_00.png}}{(b) Power Density}
% \vspace*{-8pt}
% \caption{Characteristics of a 8$\times$8 transformed DCT spectrum.}
% \vspace{-15pt}
% \label{fig:spectra}
% \end{figure}
 
 % is our main task. JPEG\cite{jpegstandard} occur block and blurry artifacts to images. We will briefly discuss the JPEG mechanism in \cref{problemformulation}.
%Before DNN methods are in the spotlight, expert rule algorithms are suggested to relieve compression artifacts such as a content-adaptive filter by A. Foi \etal\cite{sadct}, and maximum a posterior (MAP) approach by T.S. Wong \etal.

%T.S. Wong \etal \cite{jpegmapapproach} propose a method using maximum a posterior (MAP) estimation to relieve artifacts. 

% There are straightforward ways for BDE, such as zero padding (ZP) method and the bit replication (BR) \cite{ulichney1998pixel}, which sets `0' or most significant bits (MSBs) for missing bits. Even though these algorithms are hardware friendly, each reconstructed signal depends only on its value without considering surrounding pixels. In contrast, interpolation methods \cite{wan20122d,cheng2009bit}, content-adaptive (CA) BDE, and contour region reconstruction (CRR) effectively remove false contour artifacts. However, they blur the details. Intensity potential for adaptive de-quantization (IPAD) method\cite{8283657} proposed an iterative algorithm which uses the intensity potential field calculated with the connected component label. IPAD achieved higher PSNR than the algorithms above. However, IPAD still suffers from false contour artifacts in large BDE.

% \begin{figure}[t]
% \footnotesize
% \centering
% \includegraphics[width = 3.4in]{Fig/Intro/Fig_3_ver_1_00.png}
% \caption{\textbf{Overall process of the JPEG encoder.} Luminance and chroma components are separated from an RGB image. Chroma components are downsampled. Both components are converted to DCT spectra and quantized with pre-defined quantization map. All losses occur in the orange area.}
% \vspace*{-15pt}
% \label{fig:visual_demo}
% \vspace{-4pt}
% \end{figure}

% Meanwhile, the BDE is highly related to de-banding. The banding artifacts are staircase-like color phenomena of images, especially in video contents. Previous works \cite{tu2020adaptive,8759906} resolved de-banding with adaptive filter-based methods. Because the artifact is mainly derived from compression with quantization, we apply our de-quantization method to remove the banding artifact. 
% On the other hand

% \noindent{\bf Learning in the Frequency domain} Several approaches have been proposed to skip a conventional JPEG decoding in an image classification task \cite{related_taking_freq_2018_fasterneural,relatied_taking_freq_xu2020learning}, especially optimizing CNNs. However, two channels (chroma) of A DCT spectrum are downsampled. Therefore, some embedding techniques are suggested in \cite{related_taking_freq_2018_fasterneural}, such as upsampling chroma components before forwarding to a network and upsampling chroma features after forwarding to a shallow network. The suggested methods boost computation time without dropping the original performance.

%By Parseval's theorem\cite{parsevaltheorem}, the power of a image in the spatial domain and frequency domain is equal. 




% The proposed neural network algorithms \cite{byun2018bitnet,xiao2018gradient,su2019photo,liu2019calf} predict favorable HBD images with higher performance than the aforementioned expert rule systems\cite{wan20122d,8283657}. The BE-CALF\cite{liu2019calf} performs BDE by recovering residuals of LBD images. However, it only supports dedicated bit LBD images as inputs. Even though the BitNet\cite{byun2018bitnet} supports 3 to 6-bit inputs with a single model, the performance is not as good as BE-CALF. Unlike previous works, the D4 and D16 networks \cite{punnappurath2021little} employ the bit-wise classification per each missing bit-plane. However, multiple models are required for predicting each bit-plane (e.g., 4 to 8-bit BDE requires four independent models). Furthermore, \cref{fig:visual_demo} shows that the learning-based approach \cite{punnappurath2021little} is not able to remove false contours completely. Unlikely the prior works, we designed the network receiving randomly quantized LBD images with single training. 



% Recently, various tasks\cite{Occupancy_Networks,Local_Implicit_Grid_CVPR20,sitzmann2019siren} apply a multi-layer perceptron (MLP) as implicit neural representation. Although the INR parameterizes coordinates to continuous signals with memory-efficient frameworks, INR has two issues: per-scene optimization and spectral bias.
% To overcome a problem of per-scene optimization, prior works\cite{chen2021learning, lee2021local} concatenate latent features from inputs with coordinates. The spectral bias \cite{DBLP:conf/icml/RahamanBADLHBC19} induces the network to learn mainly low frequencies. Recently, in the super-resolution task, the local texture estimator (LTE)\cite{lee2021local} overcomes such spectral bias by learning high-resolution images' dominant frequency and phases. Nevertheless, there is no INR for de-quantization to our best knowledge. Therefore, we suggest INR as a function of given LBD data and amplitude coordinates calculated with input and output bit-depth. Moreover, we develop a phasor estimator so that the network avoids spectral bias. 


==> sec/3_Problem_formulation.tex <==
\section{Method}\label{problemformulation}

% \begin{figure}[t]
% \footnotesize
% \centering
% \includegraphics[width = 3.4in]{Fig/3_Problemformulation/Fig_4_ver_1_01.png}
% \caption{\textbf{Group embedding of the minimum unit of JDEC} }
% \vspace*{-15pt}
% \label{fig:jpeg_process}
% \vspace{-4pt}
% \end{figure}According to Shannon's source coding theorem\cite{shannoncapacity}, a loss is inevitable to achieve high-efficiency compression. In this section, we briefly discuss the JPEG\cite{jpegstandard} encoding algorithm and summarize the essential role of the JPEG decoder.  % Note that $\mathbf{I_Y}\sim \mathbf{I^{*}_{Y}}\in \mathbb{R}^{\frac{H}{8}\times \frac{W}{8}\times 8 \times 8 \times 1}$ where $^*$ indicates reshape.

\noindent\textbf{Problem Formulation}  Let $\mathbf{I_{GT}} \in \mathbb{R}^{H\times W \times 3}$ be a ground-truth RGB image. 
% We use tilde $\Tilde{(\cdot)}$  notation as the occurrence of loss. 
The JPEG encoder separates $\mathbf{I_{GT}}$ to luminance component ($\mathbf{I_{Y}}\in \mathbb{R}^{H\times W \times 1}$) and chroma components ($\mathbf{I_{C}}\in \mathbb{R}^{H\times W \times 2}$) and downsamples chroma components by a factor of 2, i.e. ($\mathbf{{I}^{\downarrow}_{C}}\in \mathbb{R}^{\frac{H}{2}\times \frac{W}{2} \times 2}$). The superscript $\downarrow$ indicates a $\times 2$ downsampling. Then, each component is divided into $8\times8$ blocks ($\mathbf{I} \in \mathbb{R}^{8\times8} \subset \mathbf{I_{Y}},\mathbf{{I}^{\downarrow}_{C}}$). 2D-DCT \cite{ahmed1974discrete} into spectra $\mathbf{X}\in\mathbb{R}^{8\times8}  $ is defined as below:
\begin{align}\label{eq:dct}
   DCT(\mathbf{I}) := \mathbf{X} &= \mathbf{D}\mathbf{I}\mathbf{D}^\top.
\end{align}
The orthonormal basis matrix $\mathbf{D}(=\mathbf{D}_{8})$ is defined as:
\begin{align}
      \tiny\mathbf{D}_N&:= \left[ \alpha \right] \odot \cos([\pi {[{F_{k|N}}]^{N-1}_{k=0}}\otimes [k]^{N-1^\top}_{k=0}])\\
      =&\sqrt{\frac{2}{N}}\left[\begin{smallmatrix}
         \frac{1}{\sqrt{2}}                & \frac{1}{\sqrt{2}} &\cdots  & \frac{1}{\sqrt{2}}\\
         \cos \left(\frac{1\pi}{2N}\right) &\cos \left(\frac{3\pi}{2N}\right) &\cdots &\cos \left(\frac{(2N-1)\pi}{2N}\right)\\
            \vdots &\vdots &\ddots &\vdots\\
         \cos \left(\frac{(N-1)\pi}{2N}\right) &\cos \left(\frac{3(N-1)\pi}{2N}\right) &\cdots &\cos \left(\frac{(2N-1)(N-1)\pi}{2N}\right)\\ \nonumber
     \end{smallmatrix}\right].\label{eq:orthobasis}
\end{align}
where ${F_{k|N}} := (2k+1) \slash 2N$ is a fixed frequency of a coordinate $k$ with a given size $N$ and $[\alpha]$ is the scaling matrix for orthonormality.
The operations $\otimes$ and $\odot$ are a Kronecker product and element-wise multiplication, respectively.
% \begin{equation}
% \end{equation}
% Note that the orthonormal basis $$ where $F_N$ is a set of the fixed frequency and $\delta$ is block coordinates. 


% The \cref{eq:dct} is equivalent to $\vec{\mathbf{X}} = (D\otimes D) \vec{\mathbf{I}}$, where $\otimes$ is Kronecker product and $\vec{\cdot}$ is a vectorized matrix. 
Quantization is conducted with a predefined quantization matrix $\mathbf{Q} = [\mathbf{{Q}_{Y}};\mathbf{Q_C}]\in {\mathbb{N}^{8\times8\times2}}$ s.t.
\vspace*{-5pt}
% Spectra divided with the pre-defined quantization map depending on the quality factor ($\mathbf{Q}:=[q_{u,v}]\in {\mathbb{N}^{8\times8}}$) and rounded s.t. 
\begin{equation}\label{eq:quantize_spectra}
% \vspace*{-15pt}
    \tilde{\mathbf{C}} := \left\lfloor  \mathbf{X}\odot \frac{1}{\mathbf{Q}}  \right\rceil,~
    \Tilde{\mathbf{X}} =  \tilde{\mathbf{C}}  \odot \mathbf{Q},
    % \label{eq:dequanspectra}
% \vspace*{-15pt}%and calculates \cref{eq:quantize_spectra} in the conventional decoder part.
\end{equation}
% \vspace*{-15pt}
% \noindent$\odot$ indicates an elementwise multiplication and  
where $\lfloor \cdot \rceil$ is a round operation that maps to the nearest integer. $1/\mathbf{Q}$ denotes an element-wise division. 
The JPEG encoder compresses the header $\mathbf{Q}$ and the body of a code $\tilde{\mathbf{C}}$ separately. 
In the decoder part, the JPEG restores the image from the compressed header and body by $\tilde{\mathbf{I}} = DCT^{-1}(\Tilde{\mathbf{C}} \odot \mathbf{Q})$.

 To summarize this, the corrupted JPEG image $\tilde{\mathbf{I}}$ is obtained by
\begin{align}\label{eq:overall}
 \begin{bmatrix}
    \mathbf{\Tilde{I}_{Y}} \\
   \mathbf{\Tilde{I}_{C}}
 \end{bmatrix}= \begin{bmatrix}
   DCT^{-1}(\lfloor DCT(\mathbf{I_{Y}})\odot\frac{1}{{\mathbf{Q}_Y}}\rceil\odot\mathbf{Q_Y})\\
   DCT^{-1}(\lfloor DCT(\mathbf{I^{\downarrow}_{C}})\odot\frac{1}{{\mathbf{Q}_C}}\rceil\odot\mathbf{Q_C})^{\uparrow}
 \end{bmatrix},
 % \begin{bmatrix}
 %     {\tilde{I}_Y} \\
 %      {\tilde{I}_C} 
 % \end{bmatrix}= \begin{bmatrix}
 %    (D^T\otimes D^T) (\vec{Q}\odot\lfloor\frac{1}{\vec{Q}}\odot(D\otimes D) \vec{I}_Y\rceil)\\
 %    (D^T\otimes D^T) (\vec{Q}\odot\lfloor\frac{1}{\vec{Q}}\odot(D\otimes D) \vec{I}^{\downarrow}_C\rceil)^{\uparrow}
 % \end{bmatrix}
%Q\mathbf{({X}^{\downarrow}_{Cr}})^{\uparrow}
\end{align}
% \begin{align}
% \mathbf{\tilde{I}} \sim& \left[\mathbf{\tilde{I}_Y}; \mathbf{\tilde{I}^{\uparrow}_{Cb}}; \mathbf{\tilde{I}^{\uparrow}_{Cr}}\right] \\
% \overset{\text{\cref{eq:dct}}}{\longleftrightarrow}& \left[ Q\mathbf{({X}_{Y})};Q\mathbf{({X}^{\downarrow}_{Cb})};Q\mathbf{({X}^{\downarrow}_{Cr}}) \right] 
% \end{align} where $Q(\cdot )$ is {\cref{eq:quantize_spectra}}
where 
% $(\cdot)^{\uparrow}$ 
the superscript $\uparrow$ indicates $\times2$ upsampling in the spatial domain. 
% Note that $\mathbf{\tilde{{X}}_{C}}\in \mathbb{R}^{\frac{H}{2}\times\frac{W}{2}\times2}$ while $\mathbf{\tilde{X}_Y} \in \mathbb{R}^{{H}\times{W}\times1}$. 
We here observe from \cref{eq:overall} that most of the loss of image information is induced by the quantization step.
The shape of the chroma component $\mathbf{\tilde{{X}}_{C}}\in \mathbb{R}^{\frac{H}{2}\times\frac{W}{2}\times2}$ is different from the luminance component $\mathbf{\tilde{X}_Y} \in \mathbb{R}^{{H}\times{W}\times 1}$. 
We will consider observations in the design of our proposed network.

% In designing the JPEG decoder we therefore consider 1) losses driven from \cref{eq:overall} and 2) embedding $\mathbf{\tilde{X}_Y}$ and $\mathbf{\tilde{{X}}_{C}}$ simultaneously where they have different size.

% Thus, retrieving losses from JPEG compression is equal to reconstructing 1) quantization of spectra and 2) downsamples of chroma images.Suppose that images $\mathbf{\tilde{I}, I \in \mathbb{R}^{H\times W \times 3}}$. covering all quality factors such as \cref{fig:rdcurve}, 2) 

%  Our overall model JDEC ($\mathbf{J_\Theta}$) has the following objective $^\forall \mathbf{Q}$ : 
% \begin{align}
%     \mathbf{J_{\Theta}} \colon (\mathbf{\tilde{X}_{Y},\tilde{X}_{C};Q}) \mapsto  \mathbf{\widehat{I}}.
% \end{align}
% To achieve the objective, JDEC includes the necessary conditions mentioned in \cref{sec:intro}: 1) embedding spectra and 2) restoring losses. 
% In this section, we demonstrate the components corresponding to the aforementioned conditions. 
% Our JDEC comprises three parts: encoder with group embedding, feature formulation following DCT, and trainable implicit transformation. 

%%%% Revision .... 
We propose a JPEG decoder network, {JDEC} $\mathbf{J_\Theta}$, defined by
\begin{align}
    \mathbf{J_{\Theta}} \colon 
        (\mathbf{\tilde{X}_{Y},\tilde{X}_{C};Q}) \mapsto \mathbf{\widehat{I}}.
\end{align}
The network directly accepts quantized spectrum $\mathbf{\tilde{X}_{Y}}$ and $\mathbf{\tilde{X}_{C}}$ with a quantization matrix as the network inputs, enabling to decode JPEG directly from encoded JPEG data.
% Note that the shape of the chroma component $\mathbf{\tilde{{X}}_{C}}\in \mathbb{R}^{\frac{H}{2}\times\frac{W}{2}\times2}$ is different from the luminance component $\mathbf{\tilde{X}_Y} \in \mathbb{R}^{{H}\times{W}\times 1}$. 
% In designing the JPEG decoder we will consider 1) losses driven from \cref{eq:overall} and 2) embedding $\mathbf{\tilde{X}_Y}$ and $\mathbf{\tilde{{X}}_{C}}$ simultaneously where they have different size.
Our proposed JDEC comprises mainly three parts: encoder $\mathbf{E}_{\varphi}$ with group embedding, continuous cosine formulation $\mathbf{T}_{\psi}$, and decoder $f_\theta$ with an implicit neural representation.

% To achieve the objective, we designed our network into three parts: 1) encoder with group embedding, 2) feature formulation as DCT, and 3) implicit transformation as decoder. $\mathbf{\tilde{X}_Y}\in \mathbb{R}^{\frac{H}{8} \times \frac{W}{8} \times8\times8 \times1}$ 

% \subsection{Encoder }%($\mathbf{E_\varphi}$)} \

\noindent\textbf{Encoder ($\mathbf{E_\varphi}$)} 
% As the solution of the first requirements of JDEC, we use the group embedding method introduced by \cite{rgbnomore} for SwinV2 \cite{Liu_2022_CVPR_swin2} transformer. 
The encoder is a function $\mathbf{E}_\varphi \colon (\mathbf{\tilde{X}_Y} , \mathbf{\tilde{X}_C}) \mapsto \mathbf{z} \in \mathbb{R}^{ \frac{H}{B}\times \frac{W}{B}\times C}$. 
% To achieve this, the group spectra embedding layer ($g_\phi$) is adopted so that the network reshape spectra of different sizes ($\mathbf{\tilde{X}_Y} \in \mathbb{R}^{H \times W \times 1},\mathbf{\tilde{X}_C}\in \mathbb{R}^{H/2 \times W/2 \times 2}$). 
We model the encoder $\mathbf{E}_\varphi$ by using SwinV2 \cite{Liu_2022_CVPR_swin2}.
To allow the different shape of spectrum $\mathbf{\tilde{X}_Y}$ and $\mathbf{\tilde{X}_C}$,
we apply the group spectra embedding layer $g_\phi$ proposed by \cite{rgbnomore}. The embedding layer ($g_\phi$) transforms luminance and chroma spectra through two steps. We convert $8\times8$ spectra into $B\times B$ for luma and $B/2\times B/2$ for chroma via sub-block conversion \cite{subblockconversion} in the (a) part of $g_\phi$ in \cref{Figmain}. We implement the block size $B = 4$\footnote{$B$ should be divisor or multiple of 16}. 
\vspace{-1pt}
\begin{align}
    \mathbf{X_{Y}'} &= \mathbf{D}^{*}_{B}\mathbf{(D^\top X_{Y}D)D}_{B}^{*\top}, \\
    \mathbf{X_{C}'} &= \mathbf{D}^{*}_{B/2}\mathbf{(D^\top X_{C}D)D}_{B/2}^{*\top},
\text{\vspace{-10pt}}
\end{align}
where $D^{*}_N$ indicates a block diagonal matrix with size $8\times8$.
In part (b) of \cref{Figmain}, spectra are reshaped and concatenated to $\mathbb{R}^{\frac{H}{B} \times \frac{W}{B} \times \frac{3B^2}{2}}$ which is the sum of converted size. Then initialized latent vector $\mathbf{z'} \in \mathbb{R}^{\frac{H}{B} \times \frac{W}{B} \times C}$ are conducted in (b) part of $g_\phi$. Following the prior work, \cite{liang2021swinir}, we adopt the deep feature extractor, replacing the Swin attention module with the SwinV2 attention module.

%into the following steps :

% \begin{enumerate}
%     \item Reshape each spectrum with converted size : \\
%     $X_{Y}': \mathbb{R}^{\frac{H}{8}\frac{W}{8} \times8\times8 \times1}\rightarrow \mathbb{R}^{\frac{H}{4}\frac{W}{4} \times4\times4 \times1}\rightarrow \mathbb{R}^{\frac{H}{4}\frac{W}{4} \times16}$\\
%     $X_{C}': \mathbb{R}^{\frac{H}{16}\frac{W}{16} \times8\times8 \times2}\rightarrow \mathbb{R}^{\frac{H}{4}\frac{W}{4} \times2\times2 \times2}\rightarrow \mathbb{R}^{\frac{H}{4}\frac{W}{4} \times 8}$
%     \item Concatenate and embed to the linear layer : \\
%     $ h_e ([X_{Y}' ; X_{C}']) = \mathbf{z}\in  \mathbb{R}^{\frac{H}{4}\frac{W}{4} \times C}$
%     \item Reshape the output : \\$\mathbf{z} :  \mathbb{R}^{\frac{H}{4}\frac{W}{4} \times C} \rightarrow  \mathbb{R}^{\frac{H}{4} \times \frac{W}{4} \times C}$
% \end{enumerate}
% where $h_e( \cdot ) : \mathbb{R}^{24} \mapsto \mathbb{R}^C$, and $\mathbf{z}$ is an initiated latent vector.

% (black module of \cref{Figmain}). 
%from the matrix encoder 
 % $h_q(\cdot) : \mathbb{R}^{128} \mapsto \mathbb{R}^K$ and $\delta$ as set of a 8$\times$8 coordinate.

 %To handle complex losses derived from the JPEG encoder, we propose the novel continuous cosine formulation (CCF), which implies enhanced cosine spectra. The CCF constructs a block of spectra as a function of block coordinate $\delta \in[0,\cdots, N-1]^2$. Therefore, each block has identical amplitudes and frequencies. 
 
\noindent\textbf{Continuous Cosine Formulation ($\mathbf{T}_\psi$)} 
Each 8$\times$8 JPEG block shares a distorted DCT spectrum.
% within each 8$\times$8 block.
% In other words, restoring the distortion of a single spectrum is equivalent to modifying the entire block. 
It is necessary to modify the entire block to restore the distortion of an 8$\times$8 spectrum.
To address the spectrum distortion issue,
% the distortion in spectrum originating from the JPEG encoder, as a function of block coordinates $[\delta_B \otimes \delta_B]$$[\delta^\top_B \otimes \delta_B]$
we introduce \textit{Continuous Cosine Formulation} (CCF) module, which enhances the cosine spectrum. The CCF constructs a continuous spectrum corresponding to $B\times B$ embedded block by estimating dominant frequencies and amplitudes of a cosine transform. As a result, a block has identical amplitudes and frequencies in the embedded $B\times B$ block coordinate $\delta :=\left[(i,j)\right]^{B-1}_{i,j=0} $. This allows us to restore losses the JPEG encoder introduced.

Our CCF takes a latent vector $\mathbf{z}$ from encoder $\mathbf{E_\varphi}$ and a quantization matrix $\mathbf{Q}$. The CCF $\mathbf{T}_\psi$ consists of three elements: frequency estimator $h_f \colon \mathbb{R}^C\mapsto \mathbb{R}^{2K}$, coefficient estimator $h_c \colon \mathbb{R}^C\mapsto \mathbb{R}^K$, and quantization matrix encoder $h_q \colon \mathbb{R}^{128} \mapsto \mathbb{R}^K$. Each frequency and coefficient estimator comprises sequential convolution and non-linear activation layers.
% As a method for quantization recovery, drawing inspiration from the existing dequantization network \cite{abcd}, we implement amplitude recovery method following as described below: 
As a method for quantization recovery, we implement an amplitude recovery method as described below, drawing inspiration from the existing dequantization network \cite{abcd}, 
\begin{align}
     \mathbf{\widehat{X} =C \odot Q'} \sim \cref{eq:quantize_spectra},
\end{align}  
where $\mathbf{Q}' = h_q(\mathbf{Q})$ and $\mathbf{C} = h_c(\mathbf{z})$.
%the quantization matrix encoder generates a de-quantization matrix Q', so the predicted spectrum $\hat{X}$ .... % The amplitude of a spectrum is estimated as i.e. $ \mathbf{A =C \odot Q'}$ 


We hypothesize that estimating the frequency components effectively mitigates aliasing (i.e., quantization and downsampling) derived from JPEG.
It has been demonstrated that trainable frequencies and phasors effectively mitigate upsampling and dequantization \cite{abcd,lee2022learning}. %Moreover, the frequencies of the JPEG spectrum were distorted twice: quantization and downsampling. 

% We thus formulate the CCF module to approximate the encoded features of 2D-DCT of a $B\times B$ feature of the encoder $\mathbf{E_\varphi}$:
We thus formulate the CCF module approximates $B\times B$ spectral features from the fiber of $\mathbf{z}$:
\begin{align}
    \mathbf{T}_\psi(\mathbf{z},\delta_{\mathbf{h,w}};\mathbf{Q}) =& \mathbf{\widehat{X}\otimes(\cos(\pi\mathbf{F}_{h}\otimes \delta_h)\odot \cos(\pi \mathbf{F}_{w}\otimes\delta_w))},%\\    \mathbf{T}_\psi(\mathbf{z},\mathbf{Q};\delta_{\mathbf{h,w}}) =& \mathbf{\widehat{X}\otimes(\cos(\pi\mathbf{F}_{h}\otimes \delta_h)\odot \cos(\pi \mathbf{F}_{w}\otimes\delta_w))},%\\%[\delta^\top_B \otimes \delta_B]^{H/B\times W/B}
\end{align} 
where $[\mathbf{F_h};\mathbf{F_w}]= h_f(\mathbf{z})$. $\mathbf{\delta_{h,w}}$ denotes vertical and horizontal coordinates of $\delta$. Note that $\mathbf{\widehat{X}}, \mathbf{F_{h}},\mathbf{F_{w}} \in \mathbb{R}^{K}$ are amplitude and frequencies for the spatial coordinate $\delta$, respectively. i.e. the CCF maps embedded features and block coordinates by $\mathbf{T_\psi} : (\mathbb{R}^{1\times1\times{C}},\mathbb{R}^{B\times B\times{2}})\mapsto \mathbb{R}^{B\times B\times{K}}$.

% First, as a method for quantization recovery, drawing inspiration from the existing dequantization network \cite{abcd},   (\mathbf{z},[\delta^\top_B \otimes \delta_B]) 
% % we implement enhanced amplitude following as described below:
% the quantization matrix encoder generates a de-quantization matrix Q', so the predicted spectrum $\hat{X}$ .... (\mathbf{z},\delta;\mathbf{Q})
%  \begin{equation}
%      \mathbf{\widehat{X} =C \odot Q'} \sim \cref{eq:quantize_spectra},
%  \end{equation} % The amplitude of a spectrum is estimated as i.e. $ \mathbf{A =C \odot Q'}$ 
% where $\mathbf{Q}' = h_q(\mathbf{Q})$.

\noindent\textbf{Decoder ($f_\theta$)} Our decoder $f_\theta\colon \mathbb{R}^{K}\mapsto \mathbb{R}^3$ is a local implicit neural representation function of $\{\mathbf{z},\mathbf{Q}\},\delta$. i.e. :
\begin{align}\label{eq:inr_final}
\tiny
    \mathbf{\widehat{I}} &= f_\theta(\mathbf{\widehat{X}\otimes(\cos(\pi\mathbf{F}_{h}\otimes\delta_h)\odot \cos(\pi \mathbf{F}_{w}\otimes\delta_w))}).
    % \\
    % \simeq &\sum_{u,v} \mathbf{X}_{u,v}\cos\left[ \frac{(2h+1)\pi u}{16} \right]\cos\left[ \frac{(2w+1)\pi v}{16} \right] .
\end{align}
 % The reconstructed $B\times B\times3$ block follows the approximation of \cref{eq:dct}.
 % The \cref{eq:orthobasis} is identical to the equation below:  Our JDEC shares estimated frequencies and amplitudes in the $B\times B\times3$ image blocks. 
Therefore, in the $B\times B$ block of \cref{eq:inr_final}, the estimated basis of $\mathbf{\hat{X}}$ and its reconstruction follows:
 % Since the estimated frequencies and amplitudes are shared in the $B\times B\times3$ image blocks,
% The \cref{eq:inr_final} is an approximation of \cref{eq:dct} with a trainable basis $\mathbf{\Lambda}$ : 
\begin{align}
 \mathbf{I} &= \mathbf{D^\top XD} \simeq f_\theta'(\mathbf{\Lambda_h}\mathbf{\widehat{X}'}\mathbf{\Lambda_w}),
 % \sim \mathbf{\vec{I}} \simeq& W \cdots \sigma \circ W \circ\sigma((\mathbf{D}^{\top}_2 \otimes \mathbf{D}_1)\mathbf{\vec{\widehat{X}}}), W \cdots \sigma \circ W \circ\sigma(\mathbf{\Lambda}_1\mathbf{\widehat{X}'}\mathbf{\Lambda}_2)  ReLU activations
 \vspace{-8pt}
\end{align}
where $\mathbf{\Lambda_{h,w}} = \cos([\pi \mathbf{F_{h,w}}\otimes{\mathbf{\delta_{h,w}}}])$ and $f'_\theta$ satisfy $f_\theta = f'_\theta \circ W$ for a trainable fully-connected layer $W$. With a linear layer $W$, the \cref{eq:inr_final} complete the quadratic form $\mathbf{\Lambda}_1\mathbf{\widehat{X}'}\mathbf{\Lambda}_2 = W(\mathbf{T_\psi(z,Q;\delta)})$ by including summation of features. 
%not only $\mathbf{X}$, but also wider than $8\times8$ domain .
We optimize a set of trainable parameters $\Theta := \{\varphi ;\psi;\theta \}$ with the equation below:
\begin{equation}
      \widehat\Theta = \arg\min_{\Theta} || \mathbf{I}_{GT} - \widehat{\mathbf{I}}(\mathbf{\tilde{X}_Y,\tilde{X}_C,Q} ; \Theta) ||_{1}.
  \end{equation}
  
We will demonstrate the estimated frequencies ($\mathbf{F_h},\mathbf{F_w}$) and amplitudes $\mathbf{\widehat{X}}$ of networks follows $\mathbf{X}$ in the following section.

% To summarize this, the encoder $\mathbf{E}_\varphi(\cdot, \cdot) : \mathbb{R}^{ H\times W \times 1}\times  \mathbb{R}^{ \frac{H}{2}\times \frac{W}{2} \times 2} \mapsto \mathbb{R}^{ \frac{H}{4}\times \frac{W}{4}\times C}$


 % Previous studies \cite{liang2021swinir, rgbnomore} have demonstrated that increasing the window size to 8 decreases overall network performance.

% \subsection{Feature Formulation}

% \subsection{Implicit transform}

%%%WOO-Formulate
% \begin{figure}[t]
% \footnotesize
% \centering
% \includegraphics[width = 3.4in]{Fig/3_Problemformulation/Fig_4_ver_2_02.png}
% \caption{\textbf{Overall process of the JPEG encoder.} Luminance and chroma components are separated from an RGB image. Chroma components are downsampled. Both components are converted to DCT spectra and quantized with a pre-defined quantization map. All losses occur in the orange area.}
% \vspace*{-15pt}
% \label{fig:jpeg_process}
% \vspace{-4pt}
% \end{figure}

% \textbf{Background} As Shannon's source coding theorem\cite{shannoncapacity}, a loss is inevitable to achieve high-efficiency compression. In this section, we briefly discuss the JPEG algorithm and summarize losses derived from JPEG. Our network is designed to retrieve losses directly from DCT spectra. Let $\mathbf{I_{HQ}} \in \mathbb{R}^{H\times W \times 3}$ be a high-quality image. JPEG algorithm separates luminance components ($:=\mathbf{I_{Y}}\in \mathbb{R}^{H\times W \times 1}$) and chroma components ($:=\mathbf{I_{Cb}},\mathbf{I_{Cr}}\in \mathbb{R}^{H\times W \times 1}$) from RGB images. JPEG subsamples chroma components with a 4:2:0 ratio, equivalent to the {$\times 2$ nearest downsampling} ($\downarrow$ part in \cref{fig:jpeg_process}). Then, each component is divided into $8\times8$ crop ($\mathbf{I}=[I_{h,w}], (h,w\in \{0,1,\dots,7\}$) and transformed into 2D-DCT spectra $\mathbf{X} = [x_{u,v}]$ s.t.
% \begin{align}\label{eq:dct}
%     \tiny
%     {x}_{u,v}:= \alpha_{u,v}\sum_{h,w}{I}_{h,w}\cos\left[ \frac{(2h+1)\pi u}{16} \right]\cos\left[ \frac{(2w+1)\pi v}{16} \right],
% \end{align}
% where $\alpha_{u,v}$ indicates weights for orthonormality of transform. Spectra divided with quantization map ($\mathbf{Q} :=[q_{u,v}]\in {\mathbb{N}^{8\times8}}$) and rounded s.t. 
% \begin{align}\label{eq:quantize_spectra}
%     \Tilde{x}_{u,v} = \lfloor \frac{x_{u,v}}{q_{u,v}} \rceil q_{u,v}
% \end{align}
% % and $\mathbf{X}$ be the transformed spectrum of $\mathbf{I_{HQ}}$. i.e.

% % In this section, we analyze images with modular arithmetic properties and formulate implicit neural representation as a function of amplitude. Let $\mathbf{I}_N$ and $\mathbf{I}_q$ be an HBD image and an LBD image, respectively, with bit-plane zero padding when  $q<N$. Then, the quantization equation from $\mathbf{I}_N$ to $\mathbf{I}_q$ is defined as below:
% % \vspace{-2pt}
% % \begin{align}\label{eq:bitzp}
% %     \small
% %     \mathbf{I}_q = \left\lfloor  \frac{\mathbf{I}_N}{2^{N-q}} \right\rfloor 2^{N-q},
% % \end{align}
% where $\lfloor \cdot \rceil$ is a round operation that maps to the nearest integer. JPEG compress $\mathbf{Q}$ and $\lfloor \cdot \rceil$ parts separately and calculate \cref{eq:quantize_spectra} in a decoder part. 
% To summarize this, JPEG image $\tilde{\mathbf{I}}$ is 
% \begin{align}
% \mathbf{\tilde{I}}
% \overset{\text{\cref{eq:dct}}}{\longleftrightarrow}& \left[ Q\mathbf{({X}_{Y})};Q\mathbf{({X}^{\downarrow}_{Cb})^{\uparrow}};Q\mathbf{({X}^{\downarrow}_{Cr}})^{\uparrow} \right] 
% \end{align}
% % \begin{align}
% % \mathbf{\tilde{I}} \sim& \left[\mathbf{\tilde{I}_Y}; \mathbf{\tilde{I}^{\uparrow}_{Cb}}; \mathbf{\tilde{I}^{\uparrow}_{Cr}}\right] \\
% % \overset{\text{\cref{eq:dct}}}{\longleftrightarrow}& \left[ Q\mathbf{({X}_{Y})};Q\mathbf{({X}^{\downarrow}_{Cb})};Q\mathbf{({X}^{\downarrow}_{Cr}}) \right] 
% % \end{align}
% where $Q(\cdot )$ is {\cref{eq:quantize_spectra}}, and $(\cdot)^{\uparrow}, (\cdot)^{\downarrow}$ indicates $\times2$ upsampling and downsampling in the spatial domain, respectively. Thus, retrieving losses from JPEG compression is equal to reconstructing 1) quantization of spectra and 2) downsamples of chroma images.

% \noindent\textbf{Dequantization} Following the novel work\cite{abcd} solving quantization problem, we formulate a general form of quantization,
%   \begin{align}\label{eq:quant_reform}
%     \small
%       x_{u,v} &= \tilde{x}_{u,v} + c_{u,v}q_{u,v}, \quad c_{u,v}\in \left[-\frac{1}{2} ,\frac{1}{2}\right].
%   \end{align}
% where $\mathbf{R}$ represents $\small N-q$ least significant bits (LSBs) of $\mathbf{I_N}$.

% \noindent{\bf Arbitrary Bitwise Coefficients} Our method, ABCD, aims to predict coefficient  $\mathbf{C}$ to reconstruct residual images by using the implicit neural representation (INR) as a function of latent vector and its quantizing bit-query. The INR parameterizes a continuous signal with an MLP fed by coordinates \cite{sitzmann2019siren,mildenhall2020nerf,chen2021learning}.
% We design INR ($f_\theta$) using amplitudes as an input coordinate so that it represents bit-wise coefficients $\mathbf{C}$ as continuous signals along the amplitude axis as follows:
% \vspace{-2pt}
% \begin{equation}
%         \small
%         \mathbf{C}(\mathbf{x},s) \simeq f_\theta(\mathbf{I}_q[\mathcal N(\mathbf x)], s),
% \end{equation}
% where $\mathbf x $ is a 2D coordinate in the image domain and $\mathcal{N}(\mathbf x)$ is a set of nearest pixels around the center pixel, $\mathbf x$. A decoder $f_\theta$ maps coefficient image $\widehat{\mathbf{C}}$ from domain composed with latent vector and bit-wise query; $f_\theta(z,s) :(\mathcal{Z}, \mathcal{S})\mapsto \mathcal{C}$, where $z\in \mathcal{Z}$ is a latent tensor from an encoder $E_\varphi$, $\mathcal{S}$ is set of basis $e_i$ and $\mathcal{C}$ is a space of predicted coefficient values from $f_\theta$.
% % Our method, ABCD, aims to predict coefficient  $\mathbf{C}$ to reconstruct residual images by using INR as a function of latent vector $\mathbf z$ and its quantizing bit-query $s$. Inspired from \cite{lee2021local}, a decoder $f_\theta$ maps $2^{N-q}$ coefficient image from domain composed with latent vector and bit-wise query; $f_\theta(z,s) :(\mathcal{Z}, \mathcal{S})\mapsto \mathcal{C}$, where $z\in \mathcal{Z}$ is a latent tensor from an encoder $E_\varphi$, $\mathcal{S}$ is set of basis $e_i$ and $\mathcal{C}$ is a space of predicted de-quantized values from $f_\theta$.

% \noindent \textbf{Phasor Estimator} Inspired from \cite{lee2021local, tancik2020fourfeat}, we insert phasor estimator by modifying local texture estimator \cite{lee2021local} to relax spectral bias. We demonstrate the difference between our ABCD and local texture estimator in \cref{sec:dis}. The overall system is constructed as follows: 
% \begin{gather}
%         \small
%         \widehat{\mathbf{C}}(\mathbf x,\mathbf{\mathbf{I}}_q,s;\boldsymbol{\Theta}) = f_\theta(h_\psi(\mathbf z_{\mathbf x}), s),
% \end{gather}
% where $\mathbf z=E_{\varphi}(\mathbf{\mathbf{I}}_q)$, $h_\psi(\cdot)$ denotes the phasor estimator of ABCD and $\boldsymbol{\Theta}=\{\theta,\varphi, \psi\}$ is a set of trainable parameters. Our phasor estimator ($h_\psi(\cdot)$) consists of two elements: (1) an amplitude estimator ($h_a(\cdot):\mathbb{R}^{C}\mapsto \mathbb{R}^{2K}$) and (2) a phase estimator ($h_p(\cdot):\mathbb{R}^{C}\mapsto \mathbb{R}^{2K}$). Thus, given a coordinate $\mathbf{x}\in\mathbb{R}^2$, the estimating function $h_\psi(\cdot):(\mathbb{R}^C)\mapsto \mathbb{R}^{2K}$ is defined as
% \begin{gather}
% \small
% h_\psi(\mathbf{z}_{\mathbf x})=
% \begin{bmatrix}
% \mathbf{A}^{1}_{\mathbf x}\\
% \mathbf{A}^{2}_{\mathbf x}
% \end{bmatrix}
% \odot
% \begin{bmatrix}
% \cos(\pi \boldsymbol{\Phi}^{1}_{\mathbf x})\\
% \sin(\pi \boldsymbol{\Phi}^{2}_{\mathbf x})
% \end{bmatrix},\label{eq:five}\\
% \mbox{where }\begin{bmatrix}
% \mathbf{A}^{1}_{\mathbf x}\\
% \mathbf{A}^{2}_{\mathbf x}
% \end{bmatrix}
% =h_a(\mathbf z_{\mathbf x}),~
% \begin{bmatrix}
% \mathbf{\Phi}^{1}_{\mathbf x}\\
% \mathbf{\Phi}^{2}_{\mathbf x}
% \end{bmatrix}
% =h_p(\mathbf z_{\mathbf x}),
% \end{gather}
% $\mathbf{A}^{1,2}_\mathbf{x}\in\mathbb{R}^{K}$ is an amplitude vector at $\mathbf x$, $\boldsymbol{\Phi}^{1,2}_\mathbf{x}\in\mathbb{R}^{K}$ denotes a phase vector at $\mathbf x$, and $\odot$ represents element-wise multiplication. We interpret that by observing pixels inside a receptive field (RF), ABCD with the encoder ($h_\psi \circ E_\varphi$) estimates dominant phasors accurately. Here, the size of RF is decided by the encoder ($E_\varphi$). We visually demonstrate estimated phasors in \cref{fig:phasors}.



% Given a series of $\mathcal J$ images with the different levels of quantizations between $3$ and $8$, the
% learning problem is defined as follows:
% \begin{equation}
% \small
% \widehat{\boldsymbol{\Theta}}=\arg\min_{\boldsymbol{\Theta}} \sum_{j\in\mathcal{J}}\sum_{{q}\in [3,8]} \|\mathbf{C}(\mathbf{I}_N^j)-\widehat{\mathbf{C}}(\mathbf{I}_q^j,s;\boldsymbol{\Theta})\|_2.\label{eq:three}
% \end{equation}

% \noindent{\bf Bit decoding} To retrieve de-quantized image values as in Eq.\eqref{eq:residue}, bitwise coefficients ($\mathbf C$) is multiplied with basis value $s$ and added with corresponding input value $\mathbf{I}_q$ from bitplane zero-padding. The whole process of decoding is written as follows:
% \begin{equation}
%     \hat{\mathbf I}_{N}(\mathbf{x})=\underbrace{\widehat{\mathbf{C}}(\mathbf x,\mathbf{I}_q,s;\widehat{\boldsymbol{\Theta}})\times s}_{\mathbf R}+\mathbf I_{q}(\mathbf{x})
% \label{eq:eight}
% \end{equation} 


==> sec/4_Experiments.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[trim=0 0 0 0,clip,width = 3.3in]{Fig/rdcurve/fig_jpecc.001.png} \includegraphics[trim=0 0 0 0,clip,width = 3.3in]{Fig/rdcurve/fig_jpecc.002.png}
    \includegraphics[trim=0 0 0 0,clip,width = 3.3in]{Fig/rdcurve/fig_jpecc.003.png}
    \includegraphics[trim=0 0 0 0,clip,width = 3.3in]{Fig/rdcurve/fig_jpecc.004.png}
    \caption{RD curve results on LIVE-1 \cite{Live1} (top left), ICB \cite{ICBdataset} (top right), BSDS500 \cite{B500dataset} (bottom left). We highlight the high-quality factor parts $q\in[90,100]$ in the bottom right part. We show PSNR as a measure of \textit{distortion} (higher is better). We observe that our JDEC decodes high-quality images better than other methods.}
    \label{fig:RDcurve-qual}
\end{figure*}



\begin{table*}[t]
\centering
% \footnotesize{
% \begin{tabular}{c|ccc|ccccc}
\setlength{\tabcolsep}{1.2pt}
\scriptsize{
\begin{tabular}{c|>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}
|>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}
|>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}}
Test & \multicolumn{4}{c|}{LIVE-1 \cite{Live1}} &\multicolumn{4}{c|}{BSDS500 \cite{B500dataset}} &\multicolumn{4}{c}{ICB \cite{ICBdataset}}\\
\cline{1-13}
Method & $q =10$ & $q=20$& $q=30$ & $q=40$ &  $q=10$ & $q=20$& $q=30$ & $q=40$ &  $q=10$ & $q=20$& $q=30$ & $q=40$ \\
\cline{1-2}
 %Method & \# Param & & & & & & & & & &\\
\hline\hline

\multirow{2}{*}{JPEG}  
& 25.69$|$24.20 & 28.06$|$26.49 & 29.37$|$27.84 & 30.28$|$28.84 
& 25.84$|$24.13 & 28.21$|$26.37 & 29.57$|$27.72 & 30.52$|$28.69
& 29.44$|$28.53 & 32.01$|$31.11 & 33.20$|$32.35 & 33.95$|$33.14 \\
&    0.759      &    0.841      &    0.875      &    0.894 
&    0.759      &    0.844      &    0.880      &    0.900 
&    0.753      &    0.807      &    0.833      &    0.844    \\
% \multirow{2}{*}{ARCNN\cite{arcnn}}  
% & 26.66$|$26.54 & 28.97$|$28.65 & 30.29$|$29.97 & - 
% & 26.83$|$26.65 & 29.00$|$28.53 & 30.31$|$29.85 & - 
% & 30.06$|$30.38 & 32.24$|$32.53 & 33.31$|$33.72 & -             \\
% &    0.792      &    0.860      &    0.891      & -
% &    0.783      &    0.853      &    0.887      & - 
% &    0.744      &    0.778      &    0.807      & -             \\
\multirow{2}{*}{DMCNN \cite{dmcnn}}  
& 27.18$|$27.03 & 29.45$|$29.08 & - & - 
& 27.16$|$26.95 & 29.35$|$28.84 & - & - 
& 30.85$|$\quad  -\quad\quad\quad & 32.77$|$\quad  -\quad\quad\quad & - & -              \\
&    0.810      &    0.874      & - & -  
&    0.799      &    0.866      & - & -  
&    0.796      &    0.830      & - & -            \\
\multirow{2}{*}{IDCN \cite{idcn}}  
& 27.62$|$27.32 & 30.01$|$29.49 & - & - 
& 27.61$|$27.22 & 28.01$|$25.57 & - & -
& 31.71$|$\quad  -\quad\quad\quad& 33.99$|$\quad  -\quad\quad\quad  & - & - \\
&    0.816     &    0.881    &    -     &    - 
&    0.805     &    0.873    &    -     &   - 
&    0.809     &   0.838    &    -     &    -\\
\multirow{2}{*}{Swin2SR* \cite{conde2022swin2sr} }
& \textcolor{red}{27.98}$|$\quad  -\quad\quad\quad   &   -     &    - & \textcolor{red}{32.53}$|$\quad  -\quad\quad\quad 
&   -    &   -     &    -      &   -
& \textcolor{blue}{32.46}$|$\quad  -\quad\quad\quad  &- & - & \textcolor{blue}{36.25}$|$\quad  -\quad\quad\quad  \\
&   -    &   -     &    -      &   -  
&   -    &   -     &    -      &   -  
&   -    &   -     &    -      &   -  \\
\hline
\multirow{2}{*}{DnCNN \cite{dncnn}}  
& 26.68$|$26.47 & 29.12$|$28.77 & 30.43$|$30.04 & 31.34$|$30.94 
& 26.82$|$26.53 & 29.26$|$28.74 & 30.63$|$30.02 & 31.59$|$30.92
& 29.78$|$29.71 & 31.99$|$31.90 & 32.98$|$32.89 & 33.52$|$33.42 \\
&    0.794      &    0.866      &    0.895      & 0.911
&    0.793      &    0.867      &    0.898      & 0.915
&    0.726      &    0.765      &    0.786      & 0.978             \\
\multirow{2}{*}{QGAC \cite{qgac}}  
& 27.65$|$27.43 & 29.88$|$29.56 & 31.17$|$30.77 & 32.08$|$31.64 
& 27.75$|$27.48 & 30.04$|$29.55 & 31.36$|$30.73 & 32.29$|$31.53
& 32.12$|$32.09 & 34.22$|$34.18 & 35.18$|$35.13 & 35.71$|$35.65 \\
&    \textcolor{blue}{0.819}      &    \textcolor{blue}{0.882}      &    0.908      &    0.922 
&    \textcolor{blue}{0.819}      &    \textcolor{blue}{0.884}      &    0.911      &    0.926 
&    0.814      &    0.844      &    0.859      &    0.865\\
\multirow{2}{*}{FBCNN \cite{fbcnn}}  
& \textcolor{black}{27.77}$|$\textcolor{blue}{27.51} & \textcolor{blue}{30.11}$|$\textcolor{blue}{29.70} & \textcolor{blue}{31.43}$|$\textcolor{blue}{30.92} & \textcolor{black}{32.34}$|$\textcolor{blue}{31.80} 
& \textcolor{blue}{27.85}$|$\textcolor{blue}{27.53} & \textcolor{blue}{30.14}$|$\textcolor{blue}{29.58} & \textcolor{blue}{31.45}$|$\textcolor{blue}{30.74} & \textcolor{blue}{32.36}$|$\textcolor{blue}{31.54}
& \textcolor{black}{32.18}$|$\textcolor{blue}{32.15} & \textcolor{blue}{34.38}$|$\textcolor{blue}{34.34} & \textcolor{blue}{35.41}$|$\textcolor{blue}{35.35} & \textcolor{black}{36.02}$|$\textcolor{blue}{35.95} \\
&    \textcolor{black}{0.816}    &    \textcolor{black}{0.881}      &    \textcolor{blue}{0.908}      &    \textcolor{blue}{0.923}  
&    \textcolor{black}{0.814}      &    \textcolor{black}{0.881}      &    \textcolor{black}{0.909}      &    \textcolor{black}{0.924} 
&    \textcolor{black}{0.813}      &    \textcolor{blue}{0.844}      &    \textcolor{blue}{0.859}      &    \textcolor{blue}{0.869}\\
% \multirow{2}{*}{SwinIR\cite{liang2021swinir}}  
% & 28.06$|$27.76 & 30.45$|$29.97 & 31.82$|$31.24 & 32.75$|$32.12 
% & 28.18$|$27.72 & 30.53$|$29.74 & 31.90$|$30.91 & 32.86$|$31.70
% & 32.60$|$32.58 & 34.82$|$34.78 & 35.90$|$35.84 & 36.49$|$36.32 \\
% &    0.809      &    0.874      &    0.902      &    0.917  
% &    0.807      &    0.875      &    0.904      &    0.920 
% &    0.820      &    0.847      &    0.861      &    0.870 \\
\multirow{2}{*}{\textbf{JDEC \textit{(ours)}}}  
& \textcolor{blue}{27.95}$|$\textcolor{red}{27.71} & \textcolor{red}{30.26}$|$\textcolor{red}{29.87} & \textcolor{red}{31.59}$|$\textcolor{red}{31.12} & \textcolor{blue}{32.50}$|$\textcolor{red}{31.98}
& \textcolor{red}{28.00}$|$\textcolor{red}{27.67} & \textcolor{red}{30.31}$|$\textcolor{red}{29.71} & \textcolor{red}{31.65}$|$\textcolor{red}{30.88} & \textcolor{red}{32.53}$|$\textcolor{red}{31.68} 
& \textcolor{red}{32.55}$|$\textcolor{red}{32.51} & \textcolor{red}{34.73}$|$\textcolor{red}{34.68} & \textcolor{red}{35.75}$|$\textcolor{red}{35.68} & \textcolor{red}{36.37}$|$\textcolor{red}{36.28} \\
&   \textcolor{red}{ 0.821}      &    \textcolor{red}{0.885 }     &    \textcolor{red}{0.911}      &    \textcolor{red}{0.925} 
&    \textcolor{red}{0.819}      &    \textcolor{red}{0.885}      &    \textcolor{red}{0.912}      &    \textcolor{red}{0.927} 
&   \textcolor{red}{0.818}     &    \textcolor{red}{0.847}      &    \textcolor{red}{0.862}      &    \textcolor{red}{0.871}
\end{tabular}}
\vspace*{-6pt}
\caption{Quantitative comparisons (PSNR (dB) $|$ PSNR-B (dB) (top), SSIM (bottom)) with \textit{the color JPEG artifact removal} networks. \textcolor{red}{Red} and \textcolor{blue}{blue} colors indicate the best and the second-best performance, respectively. (-) indicates not reported. (*) indicates using additional datasets. Note that only JPEG \cite{jpegstandard} and our JDEC get spectra as input.}
\label{tab:Quan_testvalid}
\end{table*}


\section{Experiments}
\subsection{Implementation Details}
\noindent \textbf{Encoder ($\mathbf{E}_\varphi$) and Decoder ($f_\theta$)} The linear layer in group spectra embedding module $g_\phi$ has an embedding size $C$ of 256. We modified the deep feature extract part of SwinIR \cite{liang2021swinir}. The window attention module is replaced with SwinV2 \cite{Liu_2022_CVPR_swin2}, with a window size of 7. 
\cite{liang2021swinir} and \cite{rgbnomore} reported that a window size of 8 significantly drops the performance of the network.  Each residual Swin transformer block includes 6 Swin transformer layers. The decoder $f_\theta$ is an MLP composed of 5 linear layers with 512 hidden channels $K$ and ReLU activations.
% subsection{Implementation Details}

\noindent \textbf{CCF} The CCF includes a frequency estimator $h_f$, an amplitude estimator $h_c$, and a quantization matrix encoder $h_q$. 
% The work of \cite{lee2021local,lee2022learning} and \cite{abcd} 
\cite{lee2021local,lee2022learning,abcd} show that learning frequency, phase, and amplitude components enhance the performance of the INR. The quantization matrix encoder $h_q$ is a single fully connected layer, having 512($=K$) channels. The amplitude and frequency estimator ($h_c, h_f$) is designed with two $3\times3$ convolutional layers with a ReLU activation. The frequency estimator has $2K (= 1024)$ output channels for $h$ and $w$ axis, while the amplitude estimator has $K (=512)$ channels. 


% \begin{table*}[t]
% \centering
% \setlength{\tabcolsep}{1.2pt}
% \scriptsize{
% \begin{tabular}{p{1.7cm}|>{\centering\arraybackslash}p{0.5cm}|>{\centering\arraybackslash}p{1.9cm}>{\centering\arraybackslash}p{1.9cm}>{\centering\arraybackslash}p{1.9cm}>{\centering\arraybackslash}p{1.9cm}>{\centering\arraybackslash}p{1.9cm}>{\centering\arraybackslash}p{1.9cm}}
% % \multicolumn{2}{c|}{Color} & \multicolumn{6}{c}{Method}\\
% % \hline
% % \centering{Dataset}&QF &JPEG & DMCNN & QGAC& FBCNN &SwinIR* & \textbf{JPECC} (Ours)\\
% % \hline\hline
% % \centering\multirow{4}{*}{Live-1}
% % &10%-----------------------------------Color-LIVE1-10----------------------
% % & 25.67
% % & 27.18 
% % & 27.62 
% % & 27.77$|$0.803$|$\textcolor{black}{27.51}
% % & \textcolor{blue}{28.06}$|$\textcolor{blue}{0.809}$|$\textcolor{blue}{27.76}
% % &\textcolor{red}{28.24}$|$\textcolor{red}{0.811}$|$\textcolor{red}{27.96}  \\                                  
% % &20 %------------------------------------Color-LIVE1-20-----------------------
% % & 28.06 
% % & 29.45 
% % & 29.88 
% % & \textcolor{black}{30.11}$|$\textcolor{black}{0.868}$|$\textcolor{black}{29.70}
% % & \textcolor{blue}{30.45}$|$\textcolor{blue}{0.874}$|$\textcolor{blue}{29.97}
% % & \textcolor{red}{30.55}$|$\textcolor{red}{0.875}$|$\textcolor{red}{30.11} \\
% % &30%------------------------------------Color-LIVE1-30-----------------------
% % & 29.37
% % & - 
% % & 31.17
% % &  \textcolor{black}{31.43}$|$\textcolor{black}{0.897}$|$\textcolor{black}{30.92}
% % & \textcolor{blue}{31.82}$|$\textcolor{blue}{0.902}$|$\textcolor{blue}{31.24}
% % & \textcolor{red}{31.88}$|$\textcolor{red}{0.903}$|$\textcolor{red}{31.35} \\
% % &40 %------------------------------------Color-LIVE1-40-----------------------
% % & 30.28 
% % & - 
% % & 32.05 
% % & {32.34}$|$0.913$|$\textcolor{black}{31.80} 
% % & \textcolor{blue}{32.75}$|$\textcolor{blue}{0.917}$|$\textcolor{blue}{32.12}
% % & \textcolor{red}{32.81}$|$\textcolor{red}{0.918}$|$\textcolor{red}{32.24} \\
% % \hline
% % \centering\multirow{4}{*}{BSDS500} 
% % &10 %------------------------------------Color-BSDS500-10-----------------------
% % & 25.82 
% % & 27.16 
% % & 27.74 
% % & \textcolor{black}{27.85}$|$\textcolor{black}{0.799}$|$\textcolor{black}{27.52}
% % & \textcolor{blue}{28.18}$|$\textcolor{blue}{0.807}$|$\textcolor{blue}{27.72} 
% % & \textcolor{red}{28.30}$|$\textcolor{red}{0.808}$|$\textcolor{red}{27.91}  \\                                  
% % &20 %------------------------------------Color-BSDS500-20-----------------------
% % & 28.21 
% % & 29.35 
% % & 30.01 
% % & \textcolor{black}{30.14}$|$\textcolor{blue}{0.867}$|$\textcolor{black}{29.56}
% % &\textcolor{blue}{30.53}$|$\textcolor{red}{0.875}$|$\textcolor{blue}{29.74}
% % & \textcolor{red}{30.57}$|$\textcolor{red}{0.875}$|$\textcolor{red}{29.92} \\
% % &30 %------------------------------------Color-BSDS500-30-----------------------
% % & 29.57 
% % & - 
% % & 31.33 
% % &  \textcolor{black}{31.45}$|$\textcolor{blue}{0.897}$|$\textcolor{black}{30.72}
% % & \textcolor{blue}{31.90}$|$\textcolor{red}{0.904}$|$\textcolor{blue}{30.91}
% % & \textcolor{red}{31.92}$|$\textcolor{red}{0.904}$|$\textcolor{red}{31.10} \\
% % &40 %------------------------------------Color-BSDS500-40-----------------------
% % & 30.52 
% % & - 
% % & 32.25 
% % & \textcolor{blue}{32.36}$|$\textcolor{blue}{0.913}$|$\textcolor{black}{31.52} 
% % & \textcolor{red}{32.86}$|$\textcolor{red}{0.920}$|$\textcolor{blue}{31.70}
% % & \textcolor{red}{32.86}$|$\textcolor{red}{0.920}$|$\textcolor{red}{31.93}\\
% % \hline
% % \centering\multirow{4}{*}{ICB} 
% % &10 %------------------------------------Color-ICB-10-----------------------
% % & 29.44 
% % & 27.16
% % & 32.11
% % & \textcolor{black}{32.18}$|$\textcolor{black}{0.815}$|$\textcolor{black}{32.15}
% % & \textcolor{blue}{32.60}$|$\textcolor{blue}{0.820}$|$\textcolor{blue}{32.58}
% % & \textcolor{red}{33.03}$|$\textcolor{red}{0.823}$|$\textcolor{red}{32.98}  \\
% % &20 %------------------------------------Color-ICB-20-----------------------
% % & 28.21 
% % & 29.35 
% % & 34.23 
% % & \textcolor{black}{34.38}$|$\textcolor{black}{0.844}$|$\textcolor{black}{34.34}
% % & \textcolor{blue}{34.82}$|$\textcolor{blue}{0.847}$|$\textcolor{blue}{34.78}
% % & \textcolor{red}{35.13}$|$\textcolor{red}{0.851}$|$\textcolor{red}{35.06} \\
% % &30 %------------------------------------Color-ICB-30-----------------------
% % & 29.57
% % & - 
% % & 35.20
% % &  \textcolor{black}{35.41}$|$\textcolor{black}{0.857}$|$\textcolor{black}{35.35}
% % & \textcolor{blue}{35.90}$|$\textcolor{blue}{0.861}$|$\textcolor{blue}{35.84}
% % & \textcolor{red}{36.18}$|$\textcolor{red}{0.867}$|$\textcolor{red}{36.09} \\
% % &40 %------------------------------------Color-ICB-40-----------------------
% % & 30.52
% % & - 
% % & 32.25
% % & \textcolor{black}{36.02}$|$\textcolor{black}{0.866}$|$\textcolor{black}{35.95}
% % & \textcolor{blue}{36.49}$|$\textcolor{blue}{0.870}$|$\textcolor{blue}{36.32}
% % & \textcolor{red}{36.83}$|$\textcolor{red}{0.879}$|$\textcolor{red}{36.73}\\
% \hline\hline
% \multicolumn{2}{c|}{Y-Channel} & \multicolumn{6}{c}{Method}\\
% \hline
% \centering{Dataset}&QF &JPEG & DMCNN & QGAC& FBCNN &SwinIR* & \textbf{JPECC} (Ours)\\
% \hline\hline
% \centering\multirow{4}{*}{Live-1} 
% &10 %-----------------------------------Gray-LIVE1-10----------------------
% & 27.77 
% & 29.73 
% & 29.53 
% & \textcolor{black}{29.75}$|$\textcolor{black}{0.825}$|$\textcolor{black}{29.39} 
% & \textcolor{blue}{29.86}$|$\textcolor{blue}{0.829}$|$\textcolor{blue}{29.50}
% &{29.71}$|$0.826$|$29.39 \\%\textcolor{red}{30.47}$|$\textcolor{red}{0.845}$|$\textcolor{red}{30.05}  \\
% & 20 %-----------------------------------Gray-LIVE1-20----------------------
% & 30.07 
% & 32.07 
% & 31.86 
% & \textcolor{black}{32.13}$|$\textcolor{black}{0.889}$|$\textcolor{black}{31.57} 
% & \textcolor{blue}{32.25}$|$\textcolor{blue}{0.891}$|$\textcolor{blue}{31.70}
% & {32.08}$|$0.889$|$31.56\\%\textcolor{red}{32.83}$|$\textcolor{red}{0.902}$|$\textcolor{red}{32.16} \\
% &30 %-----------------------------------Gray-LIVE1-30----------------------
% & 31.41 
% & -     
% & 33.23 
% & \textcolor{black}{33.54}$|$\textcolor{black}{0.916}$|$\textcolor{black}{32.83} 
% & \textcolor{blue}{33.69}$|$\textcolor{blue}{0.917}$|$\textcolor{blue}{33.01}
% & {33.49}$|$0.915$|$32.81\\%\textcolor{red}{34.26}$|$\textcolor{red}{0.926}$|$\textcolor{red}{33.43} \\
% &40 %-----------------------------------Gray-LIVE1-40----------------------
% & 32.35
% & -
% & 34.05 
% & \textcolor{black}{34.53}$|$\textcolor{black}{0.931}$|$\textcolor{black}{33.74}
% & \textcolor{blue}{34.67}$|$\textcolor{blue}{0.932}$|$\textcolor{blue}{33.88} 
% &{34.47}$|$0.930$|$33.73 \\%\textcolor{red}{35.28}$|$\textcolor{red}{0.939}$|$\textcolor{red}{34.36} \\
% \hline
% \centering\multirow{4}{*}{BSDS500}
% &10 %-----------------------------------Gray-BSDS500-10----------------------
% & 27.80
% & 29.66 
% & 29.46 
% & \textcolor{black}{29.67}$|$\textcolor{black}{0.821}$|$\textcolor{blue}{29.22} 
% & \textcolor{blue}{29.75}$|$\textcolor{blue}{0.823}$|$\textcolor{blue}{29.22}
% &{29.62}$|$0.820$|$29.19\\%$|$\textcolor{red}{0.840}$|$\textcolor{red}{29.80} \\
% &20 %-----------------------------------Gray-BSDS500-20----------------------############
% & 30.05
% & 31.91
% & 31.73 
% & \textcolor{black}{32.00}$|$\textcolor{black}{0.885}$|$\textcolor{black}{31.19} 
% & \textcolor{blue}{32.10}$|$\textcolor{blue}{0.887}$|$\textcolor{blue}{31.21}
% & {31.94}$|$0.885$|$31.17\\%\textcolor{red}{32.70}$|$\textcolor{red}{0.899}$|$\textcolor{red}{31.73} \\
% &30 %-----------------------------------Gray-BSDS500-30----------------------
% & 31.37 
% & -     
% & \textcolor{black}{33.07} 
% & \textcolor{black}{33.37}$|$\textcolor{black}{0.913}$|$\textcolor{black}{32.32}
% & \textcolor{blue}{33.50}$|$\textcolor{blue}{0.914}$|$\textcolor{blue}{32.38}
% & {33.32}$|$0.913$|$32.30\\%\textcolor{red}{34.07}$|$\textcolor{red}{0.923}$|$\textcolor{red}{32.84} \\
% &40%-----------------------------------Gray-BSDS500-40----------------------
% & 32.30
% & -    
% & 34.01
% & \textcolor{black}{34.33}$|$\textcolor{black}{0.928}$|$\textcolor{black}{33.10}
% &\textcolor{blue}{34.48}$|$\textcolor{blue}{0.929}$|$\textcolor{blue}{33.21}
% &{34.28}$|$0.928$|$33.09\\%\textcolor{red}{35.06}$|$\textcolor{red}{0.937}$|$\textcolor{red}{33.63} \\
% \hline
% \centering\multirow{4}{*}{Classic5} 
% &10%-----------------------------------Gray-Classic5-10----------------------
% & 27.82
% & 29.98
% & 29.84
% & \textcolor{red}{30.12}$|$\textcolor{red}{0.822}$|$\textcolor{red}{29.80}
% & 30.04$|$0.819$|$29.74
% & \textcolor{black}{30.00}$|$0.819$|$29.70\\%$|$\textcolor{blue}{0.821}$|$\textcolor{blue}{29.76}  \\
%  &20%-----------------------------------Gray-Classic5-20----------------------
% & 30.12
% & 32.11
% & 31.98
% & \textcolor{blue}{32.31}$|$\textcolor{red}{0.872}$|$\textcolor{blue}{31.74}
% & 32.28$|$\textcolor{blue}{0.871}$|$\textcolor{red}{31.75}
% & 32.18$|$0.871$|$31.66\\%\textcolor{red}{32.32}$|$\textcolor{red}{0.872}$|$\textcolor{black}{31.72} \\
% &30%-----------------------------------Gray-Classic5-30----------------------
% & 31.48
% & -     
% &33.22
% & \textcolor{blue}{33.54}$|$\textcolor{red}{0.894}$|$\textcolor{blue}{32.78}
% & 33.53$|$\textcolor{blue}{0.893}$|$\textcolor{red}{32.85}
% & {33.43}$|$0.893$|$32.71\\%\textcolor{red}{33.57}$|$\textcolor{red}{0.894}$|$32.77 \\
% &40%-----------------------------------Gray-Classic5-40----------------------
% & 32.43
% & -     
% & 34.05
% & \textcolor{blue}{34.35}$|$\textcolor{red}{0.907}$|$\textcolor{blue}{33.48}
% & 34.36$|$\textcolor{red}{0.907}$|$\textcolor{red}{33.57}
% & {34.26}$|$0.906$|$33.41\\%\textcolor{red}{34.40}$|$\textcolor{red}{0.907}$|$33.48
% \end{tabular}
% }
% \vspace*{-6pt}
% \caption{Quantitative comparisons (PSNR (dB)$|$ SSIM $|$ PSNR-B(dB)) for the JPEG artifact removal.  (*) denotes trained under additional datasets including BSDS500 (Train $\&$Test). \textcolor{red}{Red} and \textcolor{blue}{blue} colors indicate the best and the second-best performance, respectively.}
% \label{tab:Quan_testvalid}
% \end{table*}
% \begin{table*}[t]
% \centering
% % \footnotesize{
% % \begin{tabular}{c|ccc|ccccc}
% \setlength{\tabcolsep}{1.2pt}
% \scriptsize{
% \begin{tabular}{c|>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}
% |>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}
% |>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}>{\centering\arraybackslash}p{1.23cm}}
% Test(Y) & \multicolumn{4}{c|}{Live-1} &\multicolumn{4}{c|}{BSDS500} &\multicolumn{4}{c}{Classic 5}\\
% \cline{1-13}
% Method& 10 & 20& 30 & 40 &  10 & 20& 30 & 40 &  10 & 20& 30 & 40 \\
% \cline{1-2}
%  %Method & \# Param & & & & & & & & & &\\
% \hline\hline

% \multirow{2}{*}{JPEG}  
% & 25.69$|$24.20 & 28.06$|$26.49 & 29.37$|$27.84 & 30.28$|$28.84 
% & 25.84$|$24.13 & 28.21$|$26.37 & 29.57$|$27.72 & 30.52$|$28.69
% & 29.44$|$28.53 & 32.01$|$31.11 & 33.20$|$32.35 & 33.95$|$33.14 \\
% &    0.743      &    0.826      &    0.861      &    0.882 
% &    0.741      &    0.827      &    0.865      &    0.887 
% &    0.753      &    0.807      &    0.833      &    0.844      \\
% \multirow{2}{*}{ARCNN\cite{arcnn}}  
% & 26.66$|$26.54 & 28.97$|$28.65 & 30.29$|$29.97 & - 
% & 26.83$|$26.65 & 29.00$|$28.53 & 30.31$|$29.85 & - 
% & 30.06$|$30.38 & 32.24$|$32.53 & 33.31$|$33.72 & -             \\
% &    0.792      &    0.860      &    0.891      & -
% &    0.783      &    0.853      &    0.887      & - 
% &    0.744      &    0.778      &    0.807      & -             \\
% % \multirow{2}{*}{DnCNN\cite{dncnn}}  
% % & 25.60$|$23.53 & 27.96$|$25.77 & 29.25$|$27.10 & 30.28$|$00.00 
% % & 25.72$|$23.44 & 28.01$|$25.57 & 29.31$|$26.85 & 30.52$|$00.00
% % & 25.72$|$23.44 & 25.72$|$23.44 & 25.72$|$23.44 & 25.72$|$23.44 \\
% % &    0.8864     &    0.8844     &    0.8843     &    0.9858 
% % &    0.9857     &    0.9990     &    0.7381     &    0.8769 
% % &    0.9556     &    0.9871     &    0.0000     &    0.0000\\
% \multirow{2}{*}{QGAC\cite{qgac}}  
% & 27.62$|$27.43 & 29.88$|$29.56 & 31.17$|$30.77 & 32.05$|$31.61 
% & 27.74$|$27.47 & 30.01$|$29.53 & 31.33$|$30.70 & 32.25$|$31.50
% & 32.06$|$32.04 & 34.13$|$34.10 & 35.07$|$35.02 & 32.25$|$31.50 \\
% &    0.804      &    0.868      &    0.896      &    0.912 
% &    0.802      &    0.869      &    0.898      &    0.915 
% &    0.816      &    0.843      &    0.857      &    0.915\\
% \multirow{2}{*}{FBCNN\cite{fbcnn}}  
% & \textcolor{red}{29.75}$|$\textcolor{blue}{29.39} & \textcolor{red}{32.13}$|$\textcolor{blue}{31.57} & \textcolor{red}{33.54}$|$\textcolor{blue}{32.83} & \textcolor{red}{34.53}$|$\textcolor{blue}{33.74} 
% & \textcolor{red}{29.67}$|$\textcolor{red}{29.22} & \textcolor{red}{32.00}$|$\textcolor{red}{31.19} & \textcolor{red}{33.37}$|$\textcolor{red}{32.32} & \textcolor{red}{34.33}$|$\textcolor{red}{33.10}
% & 30.12$|$29.80 & 32.31$|$31.74 & 33.54$|$32.78 & 34.35$|$33.48 \\
% &    \textcolor{red}{0.825}      &    \textcolor{red}{0.889}      &    \textcolor{red}{0.916}      &    \textcolor{red}{0.931}  
% &    \textcolor{red}{0.821}      &    \textcolor{red}{0.885}      &    \textcolor{red}{0.913}      &    \textcolor{red}{0.928} 
% &    0.822      &    0.872      &    0.894      &    0.907\\
% % \multirow{2}{*}{SwinIR\cite{liang2021swinir}}  
% % & 28.06$|$27.76 & 30.45$|$29.97 & 31.82$|$31.24 & 32.75$|$32.12 
% % & 28.18$|$27.72 & 30.53$|$29.74 & 31.90$|$30.91 & 32.86$|$31.70
% % & 32.60$|$32.58 & 34.82$|$34.78 & 35.90$|$35.84 & 36.49$|$36.32 \\
% % &    0.809      &    0.874      &    0.902      &    0.917  
% % &    0.807      &    0.875      &    0.904      &    0.920 
% % &    0.820      &    0.847      &    0.861      &    0.870 \\
% \multirow{2}{*}{\textbf{JDEC(Ours)}}  
% & \textcolor{blue}{29.72}$|$\textcolor{red}{29.40} & \textcolor{blue}{32.09}$|$\textcolor{red}{31.58} & \textcolor{blue}{33.50}$|$\textcolor{red}{32.84} & \textcolor{blue}{34.49}$|$\textcolor{red}{33.76}
% & \textcolor{blue}{29.63}$|$\textcolor{blue}{29.20} & \textcolor{blue}{31.96}$|$\textcolor{blue}{31.18} & \textcolor{blue}{33.33}$|$\textcolor{blue}{32.31} & \textcolor{blue}{34.30}$|$\textcolor{blue}{33.09} 
% & \textcolor{blue}{30.01}$|$\textcolor{blue}{29.71} & \textcolor{blue}{32.19}$|$\textcolor{blue}{31.68} & \textcolor{blue}{33.45}$|$\textcolor{blue}{32.76} & \textcolor{blue}{34.27}$|$\textcolor{blue}{33.44} \\
% &   \textcolor{red}{ 0.826}      &    \textcolor{red}{0.889 }     &    \textcolor{red}{0.916}      &    \textcolor{blue}{0.930} 
% &    \textcolor{red}{0.821}      &    \textcolor{red}{0.885}      &    \textcolor{red}{0.913}      &    \textcolor{red}{0.928} 
% &   \textcolor{blue}{0.820}     &    \textcolor{blue}{0.871}      &    \textcolor{blue}{0.893}      &    \textcolor{blue}{0.906}
% \end{tabular}
% }
% \vspace*{-6pt}
% \caption{Quantitative comparisons (PSNR (dB)$|$ SSIM $|$ PSNR-B(dB)) for the JPEG artifact removal.  (*) denotes trained under additional datasets including BSDS500 (Train $\&$Test). \textcolor{red}{Red} and \textcolor{blue}{blue} colors indicate the best and the second-best performance, respectively. (-) indicates not reported.}
% \label{tab:Quan_testvalid}
% \end{table*}


% \begin{table}[t]
% \vspace{-6pt}
% \centering
% \setlength{\tabcolsep}{1.2pt}
% \small
% \begin{tabular}{c
% |>{\centering\arraybackslash}p{0.80cm}
% >{\centering\arraybackslash}p{0.80cm}>{\centering\arraybackslash}p{0.80cm}>{\centering\arraybackslash}p{0.80cm}
% }
% &\multicolumn{6}{c}{Input Bit $\rightarrow$ Output Bit}\\
% \cline{2-7}
% & \tiny{$3 \rightarrow 16 $}&\tiny{ $4 \rightarrow 16 $}& \tiny{$5 \rightarrow 16 $}&\tiny{$6 \rightarrow 16 $}&\tiny{ $7 \rightarrow 16 $} &\tiny{ $8 \rightarrow 16 $}\\
% \hline\hline
% ABCD & \textbf{34.57} & \textbf{41.65} &  \textbf{47.67} &\textbf{52.78}&\textbf{57.24} & \textbf{61.78}\\
% \hline
% ABCD(-P) & 34.27 & 41.25 & 47.36 & 52.60 & 57.16 & 61.70 \\
% ABCD(-S) & {34.55} & 41.58 &{47.66} & 52.77 & \textbf{57.24} & 61.76 \\
% \hline
% ABCD(+B) & 25.27 & 31.54 & 37.70 & 43.81 & 49.87 & 55.92 \\
% ABCD(+L) & 34.26 & 41.11 & 46.87 & 51.75 & 56.08 & 60.52 \\
% \end{tabular}
% \vspace*{-6pt}
% \caption{\textbf{Quantitative ablation study} of ABCD on TESTIMAGES 1200\cite{asuni2013testimages} (PSNR(dB)). Definitions of -P, -S, +B, +L are shown in \cref{sec:abl}. EDSR\cite{Lim_2017_CVPR_Workshops} is used as an encoder. }\label{tab:Quan_abl_tab}
% \vspace{-15pt}
% \end{table}


==> sec/5_training.tex <==
\subsection{Training}

\noindent \textbf{Dataset} Following the previous work \cite{qgac,fbcnn}, we use DIV2K and Flickr2K \cite{DIV2kdataset}. Each dataset contains 800 and 2650 images, respectively. For generating synthetic JPEG compression, we use the OpenCV standard \cite{opencv_library}. We compress images using randomly sampled quality factors with steps of 10 in the range [10,100]. We directly extract quantization maps $\mathbf{Q}$ and coefficients of spectra $\mathbf{\Tilde{C}}$ from JPEG files and construct spectra $\mathbf{\Tilde{X}}$, following the \cref{eq:quantize_spectra}. Since the dynamic range of spectra depends on frequency, we should normalize spectra in a range of $[-1,1]$. The quantization maps are normalized with the same normalization function. The ground truth (GT) images are prepared with a range of $[-0.5,0.5]$ because the JPEG encoder subtracts the midpoint of the image range (=128).

\noindent \textbf{Implementation Detail} 
We use $112\times112$ patches as inputs to our network. This size is chosen because it is the least common multiple of the minimum unit size of color JPEG ($16\times16$) and the window size of our Swin architecture \cite{Liu_2022_CVPR_swin2} ($7\times7$). The network is trained for 1000 epochs with batch size 16. We optimize our network by Adam \cite{DBLP:journals/corr/KingmaB14}. The learning rate is initialized as 1e-4 and decayed by factor 0.5 at $[200,400,600,800]$.

%  which graphically
\subsection{Evaluation}
\noindent \textbf{Quantitative Result} \quad For evaluation, we use LIVE-1 \cite{Live1}, testset of BSDS500 \cite{B500dataset} and ICB \cite{ICBdataset} dataset. In the aspect of the JPEG decoder, we present the rate-distortion curve to illustrate the trade-off between bits-per-pixel (bpp) and peak signal-to-noise ratio (PSNR) where quality factors in a range of $[10,100]$. We observed that BSDS500\cite{B500dataset} is saved as JPEG with a quality factor of 95. Therefore, the reported BSDS500 data is within a quality factor of 90. We compare our JDEC against existing compression artifact removal models: DnCNN \cite{dncnn}, QGAC \cite{qgac}, and FBCNN \cite{fbcnn} in \cref{fig:RDcurve-qual}. The selected models cover a relatively wide range of quality factors with a single network. We evaluate DnCNN \cite{dncnn} following the suggested method in QGAC \cite{qgac}, with channels being processed independently. Despite QGAC \cite{qgac} having a training range of $[10,100]$, it experiences a drop in performance in the range of $\left(90,100\right]$ across all datasets. FBCNN \cite{fbcnn} also exhibits a performance drop in the range of $[95,100]$ when evaluated on the LIVE-1 \cite{Live1} dataset. In comparison, JDEC outperforms all other methods, regardless of the quality factor or dataset.

Regarding JPEG artifact removal, we report PSNR, structural similarity index (SSIM), and PSNR-B for estimating de-blocking in \cref{tab:Quan_testvalid}. We include DMCNN \cite{dmcnn}, IDCN \cite{idcn}, and transformer-based Swin2SR \cite{conde2022swin2sr} as additional comparative groups since they cover a range of quality factors. Note that the Swin2SR has trained on a limited range of quality factors in a range of $[10,40]$ with additional datasets, including the train and test dataset of BSDS500 \cite{B500dataset} and Waterloo \cite{ma2017waterloo}. We partitioned the data presented in \cref{tab:Quan_testvalid} to distinguish between networks operating within limited and expansive ranges. Our JDEC shows remarkable performance compared to other methods. The maximum PSNR interval is 0.37dB on ICB for $q=10$.

In \cref{tab:high-quality-comparison}, we show the comparison of the high-quality image decoding. The $^*$ mark indicates the commonly used default quality factor of the JPEG, including OpenCV \cite{opencv_library}. As a practical decoder for JPEG, only our {JDEC} decodes the best images among other baselines, including the conventional JPEG decoder. %Decoding이 더 잘되는 것.. HQ에서 좋은 Quality를 보장함.. 

\noindent \textbf{Qualitative Result} We show color JPEG artifact removal task in \cref{fig:Qual_jpeggone}. There are two main distortions of JPEG compression: 1) lack of High-frequency components and 2) color differences. We demonstrate the effect of our JDEC in addressing the distortions in high frequencies in the first and second rows of \cref{fig:Qual_jpeggone}. While other methods suffer from aliasing, our JDEC successfully recovers the details of the butterfly's antennae. In the third and last row of \cref{fig:Qual_jpeggone}, our JDEC relieves color distortion derived from JPEG compression.


\begin{table}[t]
\scriptsize
\vspace{-6pt}
\centering
\setlength{\tabcolsep}{1.2pt}
\begin{tabular}{c
|>{\centering\arraybackslash}p{1.5cm}
|>{\centering\arraybackslash}p{1.5cm}
|>{\centering\arraybackslash}p{1.5cm}
|>{\centering\arraybackslash}p{1.5cm}
}
{Test}&\multicolumn{4}{c}{LIVE-1\cite{Live1}}\\
\hline
Method & $q=80$&$q=90$&$q=95^*$&$q=100$ \\
\hline\hline
\multirow{2}{*}{JPEG} & 34.23$|$33.45 &  36.86$|$36.45& 39.33$|$38.90  &\textcolor{blue}{43.07}$|$\textcolor{blue}{42.37}\\
&0.948 & 0.967 &0.979 &\textcolor{blue}{0.993} \\
\multirow{2}{*}{DNCNN\cite{dncnn}}   &35.01$|$34.69 & 37.29$|$36.97&  39.20$|$38.79 & 41.15$|$40.59\\
 &  0.954&  0.970&\textcolor{blue}{0.980} & 0.987\\
\multirow{2}{*}{QGAC\cite{qgac}} & 35.75$|$35.19 & 37.75$|$37.20&37.50$|$ 37.01 & 38.97$|$38.56  \\
&0.960 &0.973&\textcolor{black}{0.974}  & 0.979\\
\multirow{2}{*}{FBCNN\cite{fbcnn}}  & \textcolor{blue}{36.02}$|$\textcolor{blue}{35.41} & \textcolor{blue}{38.25}$|$\textcolor{blue}{37.68}& \textcolor{blue}{40.23}$|$\textcolor{blue}{39.65} &  42.23$|$41.52\\
& \textcolor{blue}{0.961}& \textcolor{blue}{0.974}&\textcolor{red}{0.983}& 0.990\\
\multirow{2}{*}{\textbf{JDEC} (\textit{ours})} & \textcolor{red}{36.31}$|$ \textcolor{red}{35.73} & \textcolor{red}{38.72}$|$\textcolor{red}{38.17}  & \textcolor{red}{40.41}$|$\textcolor{red}{39.90} & \textcolor{red}{45.14}$|$\textcolor{red}{44.20}\\
 & \textcolor{red}{0.963}& \textcolor{red}{0.976}&\textcolor{red}{0.983}&\textcolor{red}{0.995} \\
\hline
\hline
{Test}&\multicolumn{4}{c}{ICB\cite{ICBdataset}}\\
\hline
Method & $q=80$&$q=90$&$q=95^*$&$q=100$ \\
\hline\hline
\multirow{2}{*}{JPEG}  & {36.34$|$35.82} & 37.72$|$ 37.40& {39.17$|$39.01} &41.31$|$41.28\\
 &0.891 &  0.912&0.934&\textcolor{blue}{0.955}\\
\multirow{2}{*}{DNCNN\cite{dncnn}}  & 35.57$|$35.44 & 36.75$|$36.64 & 37.99$|$37.92 & 39.73$|$ 39.69\\
& 0.844&0.868& 0.891 & 0.915 \\
\multirow{2}{*}{QGAC\cite{qgac}} & 37.58$|$37.47 &38.34$|$38.21& 36.84$|$36.68 &37.55$|$37.48  \\
 & \textcolor{blue}{0.902}&0.919& \textcolor{black}{0.912} & 0.926\\
\multirow{2}{*}{FBCNN\cite{fbcnn}} & \textcolor{blue}{38.03}$|$\textcolor{blue}{37.91} & \textcolor{blue}{39.17}$|$\textcolor{blue}{39.03} & \textcolor{blue}{40.36}$|$\textcolor{blue}{40.22} & \textcolor{blue}{41.61}$|$\textcolor{blue}{41.52}\\
& \textcolor{blue}{0.902}& \textcolor{blue}{0.920} &\textcolor{blue}{0.938}&  \textcolor{black}{0.951}\\
\multirow{2}{*}{\textbf{JDEC} (\textit{ours})}  & \textcolor{red}{38.43}$|$\textcolor{red}{38.29} & \textcolor{red}{39.58}$|$\textcolor{red}{39.41} & \textcolor{red}{40.77}$|$\textcolor{red}{40.63}& \textcolor{red}{43.61}$|$\textcolor{red}{43.52}\\
 & \textcolor{red}{0.906}& \textcolor{red}{0.924} &\textcolor{red}{0.943}&\textcolor{red}{0.968} \\
\end{tabular}
\vspace*{-6pt}
\caption{Quantitative comparisons of high-quality images in LIVE-1 \cite{Live1} and ICB \cite{ICBdataset} datasets (PSNR$|$PSNR-B(dB)) (top), SSIM (bottom). *: Quality factor 95 is a generally used default quality factor in the JPEG encoder.}\label{tab:high-quality-comparison}
\vspace{-1pt}
\end{table}





\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}
\begin{table}[t]
\vspace{-6pt}
\centering
\setlength{\tabcolsep}{1.2pt}
\footnotesize
\begin{tabular}{c
|>{\centering\arraybackslash}p{1cm}
|>{\centering\arraybackslash}p{1cm}
|>{\centering\arraybackslash}p{1.33cm}
|>{\centering\arraybackslash}p{1.33cm}
|>{\centering\arraybackslash}p{1.33cm}
|>{\centering\arraybackslash}p{1.33cm}
}
\multirow{2}{*}{ID}&\multicolumn{2}{c|}{Method}&\multicolumn{4}{c}{Quality Factor $q$}\\
\cline{2-7}
                      &$g_\phi$-(a) & $\mathbf{T}_\psi$ &10& 20&30&40 \\
\hline\hline
$0^*$&\checkmark&\checkmark & \textbf{27.95$|$27.71} & \textbf{30.26$|$29.87} &  \textbf{31.59$|$31.12} &\textbf{32.50$|$31.98}\\
\hline
1&\checkmark&  \xmark  & 27.76$|$27.51 & 30.04$|$29.62 & 31.35$|$30.84 & 32.25$|$31.68\\
2& \xmark &\checkmark& 27.69$|$27.43 & 29.95$|$29.53 &31.25$|$30.71 & 32.14$|$31.54  \\
% \hline
3& \xmark & \xmark & 26.90$|$26.61 & 28.37$|$28.06 & 28.73$|$28.36 & 28.96$|$28.57\\
\hline
4& \checkmark & \cref{eq:lte_dft} & 27.88$|$27.64 & 30.21$|$29.83 & 31.54$|$31.07 & 32.45$|$31.93\\
\end{tabular}
\vspace*{-6pt}
\caption{\textbf{Quantitative ablation study} of JDEC on LIVE-1 \cite{Live1} (PSNR$|$PSNR-B (dB)). $*$: ID-0 is the proposed method JDEC. The definition of each ID number is shown in \cref{sec:abl}.}\label{tab:Quan_abl_tab}
\vspace{-15pt}\label{tab:Quan_abl_tab}
\end{table}


\subsection{Ablation Study}\label{sec:abl}

\noindent \textbf{Network Components }We conducted ablation studies for the main components of our proposed JDEC. The proposed method, CCF $\mathbf{T}_\psi$ contains a frequency estimator which makes JDEC learn enhanced spectra. To support this, we train JDEC without a frequency estimator, directly forwarding concatenated coordinates (ID-1). We use additional 3$\times$3 convolutional layers to have a comparable number of parameters.
The sub-block conversion is the main element of encoder $\mathbf{E}_\varphi$. The spatial area gains a degree of freedom by using the sub-block conversion of the DCT matrix. We conduct the ablation study of sub-block conversion by embedding inputs directly (ID-2 of \cref{tab:Quan_abl_tab}). The drop in performance is severe when both components are missing (ID-3 of \cref{tab:Quan_abl_tab}).

\noindent \textbf{Fourier Features} Comparing to the existing sinusoidal representation, the formulation of \cite{lee2021local} will be compatible for our CCF. The modified Fourier feature is as follows :
\begin{equation}
\mathbf{{C}}
\odot
\begin{bmatrix}
\cos(\pi ({{\mathbf{F}\cdot\delta}}+h_q({\mathbf{Q}}))\\
\sin(\pi ({{\mathbf{F}\cdot\delta}}+h_q({\mathbf{Q}}))
\end{bmatrix} .
\vspace{-6pt}\label{eq:lte_dft}
\end{equation}
We label the model using \cref{eq:lte_dft} instead of $\mathbf{T}_\psi$ as ID-4.
The rate-distortion curve of all ablation models is illustrated in \cref{fig:ablationrd}. As shown in \cref{fig:ablationrd}, the maximum gain of our CCF is 0.58dB against ID-4, where the quality factor is 100. We also observed that  ID-3, training without both the group embedding and CCF, leads to a significant performance drop as shown in \cref{fig:ablationrd}.
% JDEC is not able to train without both the group embedding and CCF in ID-3 of \cref{fig:ablationrd}.

\begin{figure}[t]
    \vspace{-15pt}
    \centering
    \includegraphics[trim=0 0 20 0,clip,width = 3.2in]{Fig/rdcurve/rd_abl_cosmetic.png}
    \caption{\textbf{Quantitative ablation study} of JDEC on LIVE-1\cite{Live1} (RD-curve), against ablation models. Our proposed JDEC achieves higher PSNR than any other models in most of the $q$ values.}
    \label{fig:ablationrd}
    \vspace{-15pt}
\end{figure}
\subsection{Continuous Cosine Spectrum}\label{sec:demo_CCF}

In this section, we demonstrate that our CCF extracts dominant frequencies and amplitudes from highly compressed JPEG spectra. The ranges of input images (8$\times$8) are highlighted with red boxes in each image. For visualization, we observe components of CCF, including estimated frequencies $\mathbf{F_h, F_w}$ and amplitudes $\mathbf{\widehat{X}}$. We scatter frequencies in 2D space and assign a color to each amplitude. We quantize the frequencies to [0, 50] with steps of 1 and interpolate to continuous values. 

 In \cref{fig:spectra}-(a), most of the high-frequency components have been removed. The estimated spectrum with CCF is centered on high-frequency components despite such circumstances. In the case of \cref{fig:spectra}-(b), the dominant components of the spectrum are focused on relatively low-frequency. Even in this case, the extracted spectrum of CCF is concentrated in the low-frequency elements as in the ground truth.

% The top of \cref{fig:spectra} shows that missing frequencies in the w-axis are filled with CCF. The bottom part shows CCF extracts more dimmed frequencies.


\begin{figure}[t]
  \footnotesize
    \centering
    \stackunder[2pt]{\includegraphics[trim=119 350 0 0,clip,width = 3.3in]{Fig/spectra/fig_jpecc_Spec_f.001.png}}{(a) High-frequency}
    \stackunder[2pt]{\includegraphics[trim=119 350 0 0,clip,width = 3.3in]{Fig/spectra/fig_jpecc_Spec_f.002.png}}{(b) Low-frequency}
    \caption{\textbf{Comparison of the estimated spectra of the Continuous Cosine Formulation (CCF).} The quality factor of input is 10. In both cases, the estimated CCF spectrum follows the spectrum of ground-truth images despite severe distortion.}
    \label{fig:spectra}
\end{figure}


==> sec/6_discussion.tex <==
\section{Discussion}

\noindent\textbf{Implicit Neural Representation} The proposed JDEC is a function of block coordinates. To demonstrate this, the model should be able to produce results when provided with coordinates that were not observed during training. Therefore, we conducted simple super-resolution experiments using the pre-trained JDEC to represent unobserved coordinates.
\begin{figure}[t]
\footnotesize
\centering
% \includegraphics[height = 1.5in,width = 3.2in]{Fig/1_Intro/I_wish_Demo_Here.png}
\stackunder[2pt]{\includegraphics[width = 0.7in]{Fig/2_Relatedwork/Demo/demo_0.png}}{Input $(q=10)$}
\stackunder[2pt]{\includegraphics[width = 0.7in]{Fig/2_Relatedwork/Demo/demo_1.png}}{JDEC + Bicubic}
\stackunder[2pt]{\includegraphics[width = 1.4in]{Fig/2_Relatedwork/Demo/demo_2.png}}{JDEC w/o Bicubic }
\caption{\textbf{$\times2$ upsampling of compressed image ($q =10$)} in Set-5 dataset. Note that JDEC upscales the image with the change of additional coordinates $\delta$ without additional training.}
\vspace*{-5pt}
\label{fig:upsample_dis}
\vspace{-4pt}
\end{figure}
\cref{fig:upsample_dis} shows that our JDEC is clearly an implicit neural representation by extracting unseen coordinates. It also demonstrates that the resolution of estimated spectra by CCF is a function of continuous frequency. We compare our upsampling results to existing networks that aim to upsample compressed images in \cref{tab:table_upsample}. We bring the numbers from \cite{li2022hst}.






\begin{table}[t]
% \vspace{-6pt}
\centering
\setlength{\tabcolsep}{1.2pt}
\footnotesize
\begin{tabular}{
c|>{\centering\arraybackslash}p{1.53cm}
|>{\centering\arraybackslash}p{1.53cm}
|>{\centering\arraybackslash}p{1.53cm}
|>{\centering\arraybackslash}p{1.53cm}
% |>{\centering\arraybackslash}p{1.33cm}
}
\hline
\multicolumn{5}{c}{ q=10, $\downarrow\times4$}\\%&\multicolumn{4}{c}{}
\hline
Concept & SR w/ JAR & SR w/ o JAR & SR w/ JAR & Decoding\\
\hline
Method &RRDB\cite{RRDB_ESRGAN}&SwinIR\cite{liang2021swinir}&HST\cite{li2022hst}&JDEC (\textit{ours}) \\
\hline\hline
  Set5  & 22.36  & 22.45  & \textcolor{red}{22.49}  & \textcolor{blue}{22.48} \\

% ABCD(+L)& & 34.26 & 41.11 & 46.87 & 51.75 & 56.08 & 60.52 \\
\end{tabular}
\vspace*{-6pt}
\caption{\textbf{Quantitative comparison} for compressed image upsampling on the Set5 \cite{set5dataset} dataset (PSNR(dB)). The JAR refers JPEG Artifact Removal.}
\vspace{-10pt}\label{tab:table_upsample}
\end{table}


\begin{figure}[t]
\footnotesize
\centering
\stackunder[2pt]{JPEG \textbf{(bpp : 0.052)}}{\includegraphics[trim= 250 0 50 0,clip,width = 1.03in]{Fig/extreme/parrots.jpg}}
\hspace{1pt}
\stackunder[2pt]{FBCNN\cite{fbcnn}}{\includegraphics[trim= 250 0 50 0 ,clip,width = 1.03in]{Fig/extreme/parrots_fbcnn.png}}%23.96
\hspace{1pt}
\stackunder[2pt]{JDEC+}{\includegraphics[trim= 250 0 50 0 ,clip,width = 1.03in]{Fig/extreme/parrots_ours.png}}%26.70(dB)
\vspace{1mm}
{22.62 (dB) \qquad \qquad \qquad 23.96 (dB) \qquad \qquad \qquad {\color{black}\textbf{26.70 (dB)}}}
\vspace{-4pt}
\caption{\textbf{Reconstruction of the extremely compressed image ($q=0$)} in LIVE-1 \cite{Live1} dataset.}
\vspace*{-5pt}
\label{fig:extreme}
\vspace{-4pt}
\end{figure}
% \cref{fig:upsample_dis} shows that our JDEC is clearly an implicit neural representation by extracting unseen coordinates. It also demonstrates that the resolution of estimated spectra by CCF is a function of continuous frequency. 


% \begin{table}[t]
% % \vspace{-6pt}
% \centering
% \setlength{\tabcolsep}{1.2pt}
% \footnotesize
% \begin{tabular}{
% c|>{\centering\arraybackslash}p{1.53cm}
% >{\centering\arraybackslash}p{1.53cm}
% >{\centering\arraybackslash}p{1.53cm}
% >{\centering\arraybackslash}p{1.53cm}
% }
% % \hline
% Method & \#Params. & Mem. (GB) & FLOPS (G) & CPU (sec) \\
% \hline
% QGAC\cite{qgac}                 & 59.41M  & -     & -       & 1.35 \\
% FBCNN\cite{fbcnn}               & 71.92M  & 0.61  & 709.97  &  1.93 \\
% \hline
% Swin2SR\cite{conde2022swin2sr}  & 11.83M  & 2.79  & 3301.50 & 59.66 \\
% JDEC (\textit{ours})            & 38.91M  & 1.76  & 1006.72 &  6.08 \\
% % ABCD(+L)& & 34.26 & 41.11 & 46.87 & 51.75 & 56.08 & 60.52 \\
% \end{tabular}
% \vspace*{-6pt}
% \caption{ Memory consumption (MB) \& computation time (sec). }
% \vspace{-10pt}\label{tab:memcon}
% \end{table}

\noindent\textbf{Extreme Reconstruction} We primarily propose a decoding network to generate high-quality images due to its practical applicability. Consequently, we pursued the network without explicitly considering the scenario of high compression ($q=0$). However, by incorporating all image quality factors within the range [0,100] with a step size of 10 during the learning process, we successfully developed a decoding method tailored for highly compressed images. We label the additional network as JDEC+. As shown in \cref{fig:extreme}, our JDEC+ recovers the highly compressed images better than image restoration models.

\noindent\textbf{Computation Time and Memory} We report a computation time in GPU (NVIDIA RTX 3090 24GB) and memory consumption. The input size is $560\times560$ for ours, while other methods have the size of $512\times512$. Our JDEC takes 224.79 ms at decoding while Swin2SR \cite{conde2022swin2sr} takes 2203.59 ms and FBCNN \cite{fbcnn} takes 71.95 ms. JDEC takes 1.76 GB of memory for decoding, while Swin2SR takes 2.79 GB, and FBCNN takes 0.61 GB. Compared to the transformer-based method, Swin2SR, we reduce computation time by 90\% and memory consumption by 63\%.

==> sec/6_discussion_camready.tex <==
\section{Discussion}


% Therefore, we conducted simple super-resolution experiments using the pre-trained JDEC to represent unobserved coordinates.
% \begin{figure}[t]
% \footnotesize
% \centering
% % \includegraphics[height = 1.5in,width = 3.2in]{Fig/1_Intro/I_wish_Demo_Here.png}
% \stackunder[2pt]{\includegraphics[width = 0.7in]{Fig/2_Relatedwork/Demo/demo_0.png}}{Input $(q=10)$}
% \stackunder[2pt]{\includegraphics[width = 0.7in]{Fig/2_Relatedwork/Demo/demo_1.png}}{JDEC + Bicubic}
% \stackunder[2pt]{\includegraphics[width = 1.4in]{Fig/2_Relatedwork/Demo/demo_2.png}}{JDEC w/o Bicubic }
% \caption{\textbf{$\times2$ upsampling of compressed image ($q =10$)} in Set-5 dataset. Note that JDEC upscales the image with the change of additional coordinates $\delta$ without additional training.}
% \vspace*{-5pt}
% \label{fig:upsample_dis}
% \vspace{-4pt}
% \end{figure}
% \cref{fig:upsample_dis} shows that our JDEC is clearly an implicit neural representation by extracting unseen coordinates. It also demonstrates that the resolution of estimated spectra by CCF is a function of continuous frequency. We compare our upsampling results to existing networks that aim to upsample compressed images in \cref{tab:table_upsample}. We bring the numbers from \cite{li2022hst}.





% \begin{table}[t]
% % \vspace{-6pt}
% \centering
% \setlength{\tabcolsep}{1.2pt}
% \footnotesize
% \begin{tabular}{
% c|>{\centering\arraybackslash}p{1.53cm}
% |>{\centering\arraybackslash}p{1.53cm}
% |>{\centering\arraybackslash}p{1.53cm}
% |>{\centering\arraybackslash}p{1.53cm}
% % |>{\centering\arraybackslash}p{1.33cm}
% }
% \hline
% \multicolumn{5}{c}{ q=10, $\downarrow\times4$}\\%&\multicolumn{4}{c}{}
% \hline
% Concept & SR w/ JAR & SR w/ o JAR & SR w/ JAR & Decoding\\
% \hline
% Method &RRDB\cite{RRDB_ESRGAN}&SwinIR\cite{liang2021swinir}&HST\cite{li2022hst}&JDEC (\textit{ours}) \\
% \hline\hline
%   Set5  & 22.36  & 22.45  & \textcolor{red}{22.49}  & \textcolor{blue}{22.48} \\

% % ABCD(+L)& & 34.26 & 41.11 & 46.87 & 51.75 & 56.08 & 60.52 \\
% \end{tabular}
% \vspace*{-6pt}
% \caption{\textbf{Quantitative comparison} for compressed image upsampling on the Set5 \cite{set5dataset} dataset (PSNR(dB)). The JAR refers JPEG Artifact Removal.}
% \vspace{-10pt}\label{tab:table_upsample}
% \end{table}



% \cref{fig:upsample_dis} shows that our JDEC is clearly an implicit neural representation by extracting unseen coordinates. It also demonstrates that the resolution of estimated spectra by CCF is a function of continuous frequency. 


% \begin{table}[t]
% % \vspace{-6pt}
% \centering
% \setlength{\tabcolsep}{1.2pt}
% \footnotesize
% \begin{tabular}{
% c|>{\centering\arraybackslash}p{1.53cm}
% >{\centering\arraybackslash}p{1.53cm}
% >{\centering\arraybackslash}p{1.53cm}
% >{\centering\arraybackslash}p{1.53cm}
% }
% % \hline
% Method & \#Params. & Mem. (GB) & FLOPS (G) & CPU (sec) \\
% \hline
% QGAC\cite{qgac}                 & 59.41M  & -     & -       & 1.35 \\
% FBCNN\cite{fbcnn}               & 71.92M  & 0.61  & 709.97  &  1.93 \\
% \hline
% Swin2SR\cite{conde2022swin2sr}  & 11.83M  & 2.79  & 3301.50 & 59.66 \\
% JDEC (\textit{ours})            & 38.91M  & 1.76  & 1006.72 &  6.08 \\
% % ABCD(+L)& & 34.26 & 41.11 & 46.87 & 51.75 & 56.08 & 60.52 \\
% \end{tabular}
% \vspace*{-6pt}
% \caption{ Memory consumption (MB) \& computation time (sec). }
% \vspace{-10pt}\label{tab:memcon}
% \end{table}
\noindent\textbf{Implicit Neural Representation} As discussed in \cref{sec:related} and \cref{eq:overall}, a JPEG encoder downsamples chroma components. Therefore, the JPEG decoder should map: $\mathbb{R}^{\frac{H}{2}\times\frac{W}{2}\times 2} \mapsto \mathbb{R}^{H\times W\times 2}$ for chroma. Our JDEC addresses this issue through CCF ($T_\psi$) by embedding $\delta$ into $1\times1$-sized features, making the proposed JDEC a function of $\delta$. Our model is able to decode high-resolution images when provided with dense coordinates that were not observed during training. We show the advanced additional upsampling results in the supplement material.

% To demonstrate this, the model should be able to produce results when provided with coordinates that were not observed during training. We show the advanced additional upsampling results in supplement material.

\noindent\textbf{Extreme Reconstruction} We primarily propose a decoding network to generate high-quality images due to its practical applicability. Consequently, we pursued the network without explicitly considering the scenario of high compression ($q=0$). However, by incorporating all image quality factors within the range [0,100] with a step size of 10 during the learning process, we successfully developed a decoding method tailored for highly compressed images. We label the additional network as JDEC+. As shown in \cref{fig:extreme}, our JDEC+ recovers the highly compressed images better than image restoration models.

\begin{figure}[t]
\footnotesize
\centering
\stackunder[2pt]{JPEG \textbf{(bpp : 0.052)}}{\includegraphics[trim= 250 0 50 0,clip,width = 1.03in]{Fig/extreme/parrots.jpg}}
\hspace{1pt}
\stackunder[2pt]{FBCNN\cite{fbcnn}}{\includegraphics[trim= 250 0 50 0 ,clip,width = 1.03in]{Fig/extreme/parrots_fbcnn.png}}%23.96
\hspace{1pt}
\stackunder[2pt]{JDEC+}{\includegraphics[trim= 250 0 50 0 ,clip,width = 1.03in]{Fig/extreme/parrots_ours.png}}%26.70(dB)
\vspace{1mm}
{22.62 (dB) \qquad \qquad \qquad 23.96 (dB) \qquad \qquad \qquad {\color{black}\textbf{26.70 (dB)}}}
\vspace{-4pt}
\caption{\textbf{Reconstruction of the extremely compressed image ($q=0$)} in LIVE-1 \cite{Live1} dataset.}
\vspace*{-0pt}
\label{fig:extreme}
\vspace{-4pt}
\end{figure}

\noindent\textbf{Computation Time and Memory} In \cref{tab:model_complexity}, we report computational resources including the number of parameters, memory consumption, floating-point operations (FLOPs), and computational time in GPU (NVIDIA RTX 3090 24GB). The input size is $560\times560$ for ours, while other methods have the size of $512\times512$. 
%Our JDEC takes 224.79 ms at decoding while Swin2SR \cite{conde2022swin2sr} takes 2203.59 ms and FBCNN \cite{fbcnn} takes 71.95 ms. JDEC takes 1.76 GB of memory for decoding, while Swin2SR takes 2.79 GB, and FBCNN takes 0.61 GB. Compared to the transformer-based method, Swin2SR, we reduce computation time by 90\% and memory consumption by 63\%.
% \begin{figure}[h]
%     \footnotesize
%     \centering
%     \vspace{-12pt}
%     \hspace{-5pt}
%     \includegraphics[trim={0 0 0 0},clip,width=3.0in]{Rebuttal_figs/flops_vs_psnr_2.png}
%     % \includegraphics[trim={10 0 0 370},clip,width=3.0in]{Rebuttal_figs/main_fig_reb.png}
%     \vspace{-15pt}
%     \caption{FLOPs and PSNR Comparison with other methods in ICB\cite{ICBdataset} ($q=10$).}
%     \vspace{-15pt}
% \end{figure}
\begin{table}[t]
\vspace{-5pt}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.2pt}
    \begin{tabular}{c
        |>{\centering\arraybackslash}p{0.9cm}
        |>{\centering\arraybackslash}p{0.9cm}
        |>{\centering\arraybackslash}p{0.9cm}
        |>{\centering\arraybackslash}p{0.9cm}
        |>{\centering\arraybackslash}p{1.23cm}
        |>{\centering\arraybackslash}p{1.23cm}
        }
          &\#Params.& {Mem.} & {Time} &FLOPs & \multicolumn{2}{c}{PSNR$|$PSNR-B (dB)} \\
        \cline{1-1} \cline{6-7}
         Method &(M)&(GB)&(ms)& (G) &$q=10$&$q=40$\\ 
        \hline\hline
         FBCNN \cite{fbcnn}   & 70.1          & \cellcolor[HTML]{EFEFEF}\textbf{0.61} & {71.95}       &709.97           & 32.18$|$32.15               &36.02$|$35.95\\
         % JDEC(2) & 43.4M & 0.95 & 79.32& 758.10 &27.84$|$27.60&32.39$|$32.35\\
         % \hline
         % \hline
         % FBCNN+\cite{fbcnn} & 210.3 & 1.68 & 218.58 &2101.15&\textcolor{black}{32.35}$|$\textcolor{black}{32.31} &36.20$|$36.11\\
         %  JDEC-CNN+ & \cellcolor[HTML]{EFEFEF}\textbf{54.6} & \cellcolor[HTML]{EFEFEF}\textbf{1.62} & \cellcolor[HTML]{EFEFEF}\textbf{111.65}& \cellcolor[HTML]{EFEFEF}\textbf{1086.87} &\cellcolor[HTML]{EFEFEF}\textbf{32.43}$|$\cellcolor[HTML]{EFEFEF}\textcolor{blue}{\textbf{32.39}}&\cellcolor[HTML]{EFEFEF}\textcolor{blue}{\textbf{36.30}}$|$\cellcolor[HTML]{EFEFEF}\textcolor{blue}{\textbf{36.19}}\\
        % \hline
        % \hline
         Swin2SR \cite{conde2022swin2sr}  & 11.5$\leq$ & 2.79 &2203.59&3301.5&\textcolor{black}{32.46}$|$\quad  -\quad\quad\quad &\textcolor{black}{36.25}$|$\quad  -\quad\quad\quad \\
         JDEC& 38.9 & 1.76 & 224.79& {1006.72} &\cellcolor[HTML]{EFEFEF}\textbf{\textcolor{black}{32.55}}$|$\cellcolor[HTML]{EFEFEF}\textbf{\textcolor{black}{32.51}}&\cellcolor[HTML]{EFEFEF}\textbf{\textcolor{black}{36.37}}$|$\cellcolor[HTML]{EFEFEF}\textbf{\textcolor{black}{36.28}} \\
       JDEC-CNN$^\dagger$ & \cellcolor[HTML]{EFEFEF}\textbf{26.2} & 0.81          & \cellcolor[HTML]{EFEFEF}\textbf{56.59}& \cellcolor[HTML]{EFEFEF}\textbf{476.33} &{32.31}$|${32.27}&{36.19}$|${36.09}\\
    \end{tabular}
    \vspace*{-6pt}
    \caption{Computational resources \& performance comparison for a $560\times 560$ pixels in ICB \cite{ICBdataset}. $\dagger: $We replace the deep feature extractor of \cref{Figmain} with a CNN structure for comparison with the CNN-based model \cite{fbcnn}. }
    \label{tab:model_complexity}
    \vspace{-20pt}
\end{table}



 % Illustrated in Figure \ref{fig:graphical}  by embedding $\delta$ into $1\times1$-sized features. by embedding $\delta$ into $1\times1$-sized features.
